A Tight Parallel Repetition Theorem for Partially Simulatable Interactive Arguments via Smooth KL-Divergence

Hardness amplification is a central problem in the study of interactive protocols. While ``natural'' parallel repetition transformation is known to reduce the soundness error of some special cases of interactive arguments: three-message protocols and public-coin protocols, it fails to do so in the general case. The only known round-preserving approach that applies to all interactive arguments is Haitner's random-terminating transformation [SICOMP '13], who showed that the parallel repetition of the transformed protocol reduces the soundness error at a weak exponential rate: if the original $m$-round protocol has soundness error $1-p$, then the $n$-parallel repetition of its random-terminating variant has soundness error $(1-p)^{p n / m^4}$ (omitting constant factors). Hastad et al. [TCC '10] have generalized this result to partially simulatable interactive arguments, showing that the $n$-fold repetition of an $m$-round $\delta$-simulatable argument of soundness error $1-p$ has soundness error $(1-p)^{p \delta^2 n / m^2}$. When applied to random-terminating arguments, the Hastad et al. bound matches that of Haitner. In this work we prove that parallel repetition of random-terminating arguments reduces the soundness error at a much stronger exponential rate: the soundness error of the $n$ parallel repetition is $(1-p)^{n / m}$, only an $m$ factor from the optimal rate of $(1-p)^n$ achievable in public-coin and three-message arguments. The result generalizes to $\delta$-simulatable arguments, for which we prove a bound of $(1-p)^{\delta n / m}$. This is achieved by presenting a tight bound on a relaxed variant of the KL-divergence between the distribution induced by our reduction and its ideal variant, a result whose scope extends beyond parallel repetition proofs. We prove the tightness of the above bound for random-terminating arguments, by presenting a matching protocol.

==> BoundingBadEvents.tex <==
\newcommand{\ddelta}{\delta}
\newcommand{\bbeta}{\beta}
\newcommand{\hbeta}{\widehat{\bbeta}}
\newcommand{\jmp}{u}

\section{Bounding the Probability of Failure in \texorpdfstring{$\wIdl$}{hat(P)}}\label{section:BoundingBadEvent}
In this section, we prove \cref{lemma:all-Bs-are-1}, restated for convenience below.


\begin{lemma}[Restatement of \cref{lemma:all-Bs-are-1}]\label{lemma:all-Bs-are-1Rem}
	\AllBsAreOneLemma
\end{lemma}


In the following, let $\eps, k, m, \ell, \cw, W, \Unf, \wIdl$ be as in \cref{lemma:all-Bs-are-1} and let $\Idl$ and $\Rll$ be the distributions from \cref{def:Ideal,def:tReal} (respectively) with respect to $k, m, \ell, \cw$.

In \cref{sec:bad_events:def-and-main-claim} we state \cref{lemma:bad_events:main-lemma} which captures the heart of the proof of \cref{lemma:all-Bs-are-1}. In \cref{sec:bad_events:proving-lemma} we prove \cref{lemma:all-Bs-are-1} using \cref{lemma:bad_events:main-lemma} and in \cref{sec:bad_events:proving-main-lemma} we prove \cref{lemma:bad_events:main-lemma}.

\remove{
\cref{sec:bad_events:def} we define typical values of the distribution $\Idl$ and prove that they happen with high probability (\wrt $\Idl$). In \cref{sec:bad_events:extension_bits}, we use the latter to lower bound the probability that the different types of the extension bits in $\wIdl$ are all ones, yielding the proof of \cref{lemma:all-Bs-are-1Rem}.}


\subsection{Bounding the Number of Bad Columns in \texorpdfstring{$\Idl$}{P}}\label{sec:bad_events:def-and-main-claim}
\remove{\Inote{throughout, coin the term Column for the different verifiers in the $k$-fold execution }}

In order to give a formal statement for our main lemma, we broadly use the definitions of $\set{\rho_{j,i}}_{j=0}^{m+1}$, $\set{\beta_{j,i}}_{j=2}^{m+1}$, $\set{\aval_{j,i}}_{j=0}^{m+1}$, $\set{\delta_j}_{j=0}^{m+1}$ given in \cref{fig:measurements} (\cref{sec:the-smooth-extentions}) and the definitions of $\set{\ISet_{x_{<j}^k}}_{j=1}^{m+1}$, $\GSet$, $\set{\GSet_{z^k x_{<j}^k}}_{j=1}^{m+1}$, $\cZ_i$, $\cD$ given in \cref{fig:sets} (\cref{sec:the-smooth-extentions}), and in addition we define new sets and variables (\cref{fig:bad_events:gamma,fig:bad_events:add_sets,fig:bad_events:spec_rounds}) which are also broadly used, and an intuition for their purpose is given below.\remove{In particular, we define the typical values with respect to each measurement (the $\set{\rho_{j,i}}$ and $\set{\aval_{j,i}}$ measurements given in \cref{fig:measurements}, and the new measurements $\set{\gamma_{j,i}}$ which are defined below).}

%For $j \in [m+1]$ and $\tau_j = z^k x^k_{<j} \in \Supp(\Idl_{Z^k X^k_{<j}})$, 
The following definitions are with respect to some fixing of $j \in [m+1]$ and $\tau_j = z^k x^k_{<j} \in \Supp(\Idl_{Z^k X^k_{<j}})$.

\begin{figure}[h!]
	\begin{minipage}{\linewidth}
		\begin{align*}
		Z^k X^{(m+1)\times k} |  (Z^k X^k_{<j} = \tau_j) = \begin{bmatrix} z^k \\ x^k_1 \\ x^k_2 \\.\\.\\ x^k_{j-1}\\ X^k_j  \\ .\\.\\ X^k_{m+1}\end{bmatrix} 
		= \begin{bmatrix} z_{1}  & z_{2} & \ldots & z_{k} \\ x_{1,1}  & x_{1,2} & \ldots & x_{1,k}\\ 
		x_{2,1}  & x_{2,2} & \ldots & x_{2,k}\\ 
		. & . && . \\ . & . && . \\  x_{j-1,1}  & x_{j-1,2} & \ldots & x_{j-1,k}\\ X_{j,1}  & X_{j,2} & \ldots & X_{j,k} \\ . & . && . \\ . & . && . \\ X_{m+1,1}  & X_{m+1,2} & \ldots & X_{m+1,k}\end{bmatrix}
		\end{align*}
	\end{minipage}
	\caption{A matrix representation of the random coins $Z^k X^{(m+1)\times k}$ at the beginning of round $j$ conditioned on $Z^k X^k_{<j} = \tau_j$ for some $j \in [m+1]$ and $\tau_j = z^k x^k_{<j} \in \Supp(\Idl_{Z^k X^k_{<j}})$ (lowercase letter represents a fixed value and an uppercase for a radnom variable which hasn't been determined yet).}
\end{figure}

First, in  \cref{fig:bad_events:gamma} we define $\gamma_{j,i}(\tau_j)$ which measures how much
$\Idl_{X_{j,i} | Z^k X_{<j}^k}(1 | \tau_j)$ is far from
$\zfrac1{m}$ (note that this is different from $\rho_{j,i}(\tau_j)$ which measures the probability according to the next round
bit $X_{j+1,i}$ and not according to the current round's bit $X_{j,i}$). Next, we split
the set of ``good'' columns $\GSet_{\tau_j}$ (defined in \cref{fig:sets}) into the sets  $\GSet^{\rho}_{\tau_j}$ and $\GSet^{\aval}_{\tau_j}$ that satisfy
$\GSet_{\tau_j} = \GSet^{\rho}_{\tau_j} \cap \GSet^{\aval}_{\tau_j} \cap \GSet$
($\GSet$ is also defined in \cref{fig:sets}) and define a similar set
$\GSet^{\gamma}_{\tau_j}$ with respect to the $\set{\gamma_{j,i}}$ measurements
(see \cref{fig:bad_events:add_sets} for formal definitions). In addition, we
define $\jmp^{\gamma}_i(\tau_j), \jmp^{\rho}_i(\tau_j), \jmp^{\aval}_i(\tau_j)$ that outputs the first round $j' \in [j]$ (with respect to
a column $i \in [k]$) which has unexpected large jump in the value of the measurement. Note that if
$1 \in x_{<j',i}$ (\ie the \ith verifier is not active at the beginning of round
$j'$) then by definition, $\gamma_{j',i} = \rho_{j',i} = -1$ since $X_{j,i} = X_{j+1,i} = 0$ (with probability $1$) in this case. Therefore, we
define it as follows: $\jmp^{\gamma}_i(\tau_j)$ outputs the first round
$j' \in [j]$ such that $1 \notin x_{<j',i}$ (equivalently,
$i \in \ISet_{x^k_{<j'}}$ meaning that $i$ is ``active'' at round $j$) but still has an unexpected large jump in the value
of $\size{\gamma_{j',i}}$, where in case no such $j'$ exists it outputs
$\infty$. Similarly, we define $\jmp^{\rho}_i$ and $\jmp^{\aval}_i$ for the $\rho_{j',i}$ and $\aval_{j',i}$ measurements (respectively), and define
$\jmp_i$ to be the first round $j' \in [j]$ which has large jump in the value of (at least) one of the
measurements: $\gamma_{j',i}$, $\rho_{j',i}$ or $\aval_{j',i}$. Finally, for $\nu \in \set{\gamma,\rho,\aval}$ we define $\jumps^{\nu}(\tau_j)$ to be the number of columns $i \in [k]$ which have large jumps in the $\set{\nu_{j,i}}$'s measurements (\ie with $\jmp^{\nu}_i(\tau_j) < \infty$) and define $\jumps(\tau_j)$ to be the number of columns $i \in [k]$ with a jump in any of the measurement (\ie with $\jmp_i(\tau_j) < \infty$). See
\cref{fig:bad_events:spec_rounds} for the formal definitions.

\begin{table}[ht]
	\begin{center}
		\caption{\label{fig:bad_events:gamma} The $\gamma_{j,i}$ measurement}
		\begin{tabular}{|c|c|c|}
			\hline
			\textit{Definition} & \textit{Value}\\
			\hline
			$\gamma_{j,i}(\tau_j)$ & $m \cdot \Idl_{X_{j,i} | Z^k X_{<j}^k}(1 | \tau_j) - 1$\\
			\hline
		\end{tabular}
	\end{center}
\end{table}

\begin{table}[ht]
	\begin{center}
		\caption{\label{fig:bad_events:add_sets} the typical columns for each measurement}
		\begin{tabular}{|c|c|c|}
			\hline
			\textit{Definition} & \textit{Value}\\
			\hline
			$\GSet_{\tau_j}^{\gamma}$ & $\set{i \in [k] \colon \forall j'\in [j]. \size{\gamma_{j',i}} \leq 0.1}$\\
			\hline
			$\GSet_{\tau_j}^{\rho}$ & $\set{i \in [k] \colon \forall j'\in [j]. \size{\rho_{j',i}} \leq 0.1}$\\
			\hline
			$\GSet_{\tau_j}^{\aval}$ & $\set{i \in [k] \colon \forall j'\in [j]. \aval_{j',i} \in [0.01,10]}$\\
			\hline
		\end{tabular}
	\end{center}
\end{table}



An important
observation of the above is that the following holds:
\begin{enumerate}[(a)]
	\item $\GSet_{\tau_j} = \GSet^{\rho}_{\tau_j} \cap \GSet^{\aval}_{\tau_j} \cap \GSet$.
	\item $\forall \nu \in \set{\gamma, \rho, \aval}.$ $i \in \GSet^{\nu}_{\tau_j} \iff \paren{i \in \ISet_{x_{<j}^k}} \land \paren{\jmp^{\nu}_i(\tau_j) = \infty}$.
	\item $\paren{i \in \ISet_{x_{<j}^k} \cap \GSet} \land \paren{\jmp_i(\tau_j) = \infty} \iff  i \in \GSet^{\gamma}_{\tau_j} \cap \GSet^{\rho}_{\tau_j} \cap \GSet^{\aval}_{\tau_j} \cap \GSet \implies i \in \GSet_{\tau_j}$.\label{item:bad_events:start_prop:belongness}
	\item $\size{\GSet_{\tau_j}} \geq \size{\ISet_{x_{<j}^k}} - (k-\size{\GSet}) - \jumps(\tau_j)$.\label{item:bad_events:start_prop:size_bound}
\end{enumerate}
Note that we can interpret  (\ref{item:bad_events:start_prop:belongness}) as follows: if we have a column $i \in [k]$ which is ``active'' (i.e. $i \in \ISet_{x_{<j}^k}$, or equivalently, $1 \notin x_{<j,i}$), and it belongs to $\GSet$ --- the set of ``good'' columns at the beginning, and it has no unexpected jump (\ie $\jmp_i(\tau_j) = \infty$), then it holds that $i \in \GSet_{\tau_j}$ (\ie $i$ is a ``good'' column in round $j$). In addition, note that  (\ref{item:bad_events:start_prop:size_bound}) simply follows by (\ref{item:bad_events:start_prop:belongness}) since $\size{\ISet_{x_{<j}^k} \cap \GSet} \geq \size{\ISet_{x_{<j}^k}} - (k - \size{\GSet})$.

Using the above definitions, we can finally state our main lemma of this section.

%\def\BadEventMainLemma{
%	For any constant $\lambda > 0$, there exists a constant $\lambda' > 0$ such that the following holds:
%	let $k,m,\ell,\cW,\eps$ be as in \cref{lemma:all-Bs-are-1}, let $\Idl$ be the distribution from \cref{def:Ideal}, let $\GSet,\cD$ be the sets from $\cref{fig:sets}$ and let $\jumps$ be the function from \cref{fig:bad_events:spec_rounds}. Assume that at least one of the following holds:
%	\begin{enumerate}
%		\item $\size{\cD} \leq (1-\zfrac{\eps}{\lambda}) k\cdot 2^{\ell}$, or \label{item:bad_events:main-claim:D}
%		\item $\eex{\Idl}{\jumps(Z^k X^{(m+1) \times k})} \geq \zfrac{\eps k}{\lambda}$,\label{item:bad_events:main-claim:jumps}
%	\end{enumerate}
%	then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
%}


\begin{restatable}{lemma}{BadEventMainLemma}[Bounding the number of bad columns in $\Idl$]\label{lemma:bad_events:main-lemma}
	For any constant $\lambda > 0$, there exists a constant $\lambda' > 0$ such that the following holds:
	let $k,m,\ell,\cW,\eps$ be as in \cref{lemma:all-Bs-are-1}, let $\Idl$ be the distribution from \cref{def:Ideal}, let $\GSet,\cD$ be the sets from $\cref{fig:sets}$ and let $\jumps$ be the function from \cref{fig:bad_events:spec_rounds}. Assume that at least one of the following holds:
	\begin{enumerate}
		\item $\size{\cD} \leq (1-\zfrac{\eps}{\lambda}) k\cdot 2^{\ell}$, or \label{item:bad_events:main-claim:D}
		\item $\eex{\Idl}{\jumps(Z^k X^{(m+1) \times k})} \geq \zfrac{\eps k}{\lambda}$,\label{item:bad_events:main-claim:jumps}
	\end{enumerate}
	then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{restatable}

Namely, \cref{lemma:bad_events:main-lemma} implies the following: if $\Unf[W]$ is high enough, then most of the pairs $(i,z_i) \in [k] \times \zo^{\ell}$ must be ``good'' (\ie in $\cD$), and in expectation over $P$, most of the columns $i \in [k]$ should not have large jumps during the execution, (\ie $\eex{\Idl}{\jumps(Z^k X^{(m+1) \times k})}$ should be small). 

\cref{lemma:bad_events:main-lemma} is used in \cref{sec:bad_events:proving-lemma} to prove \cref{lemma:all-Bs-are-1}, and in \cref{sec:bad_events:proving-main-lemma} we prove \cref{lemma:bad_events:main-lemma}.

\begin{table}[ht]
	\begin{center}
		\caption{\label{fig:bad_events:spec_rounds} first rounds with untypical measurement.}
		\begin{tabular}{|c|c|c|}
			\hline
			\textit{Definition} & \textit{Value}\\
			\hline
			&\\
			$\jmp^{\size{\gamma} > c}_i(\tau_j)$ & $\begin{cases} \infty & \forall j' \in [j]:\text{ } \paren{\size{\gamma_{j',i}} \leq c} \lor \paren{1 \in x_{<j',i}} \\ \min\set{j' \in [j] \colon \paren{\size{\gamma_{j',i}} > c} \land \paren{1 \notin x_{<j',i}}} & \text{Otherwise}\end{cases}$\\
			&\\
			\hline
			$\jmp^{\gamma}_i(\tau_j)$ & $\jmp^{\size{\gamma} > 0.1}_i(\tau_j)$\\
			\hline
			&\\
			$\jmp^{\size{\rho} > c}_i(\tau_j)$ & $\begin{cases} \infty & \forall j' \in [j]:\text{ } \paren{\size{\rho_{j',i}} \leq c} \lor \paren{1 \in x_{<j',i}} \\ \min\set{j' \in [j] \colon \paren{\size{\rho_{j',i}} > c} \land \paren{1 \notin x_{<j',i}}} & \text{Otherwise}\end{cases}$\\
			&\\
			\hline
			$\jmp^{\rho}_i(\tau_j)$ & $\jmp^{\size{\rho} > 0.1}_i(\tau_j)$\\
			\hline
			&\\
			$\jmp^{\aval}_i(\tau_j)$ & $\begin{cases} \infty & \forall j' \in [j]: \paren{\aval_{j',i} \in [0.01,10]} \lor \paren{1 \in x_{<j',i}} \\ \min\set{j' \in [j] \colon \paren{\aval_{j',i} \notin [0.01,10]} \land \paren{1 \notin x_{<j',i}}}& \text{Otherwise}\end{cases}$\\
			&\\
			\hline
			$\jmp_i(\tau_j)$ & $\min\set{\jmp^{\gamma}_i(\tau_j), \jmp^{\rho}_i(\tau_j), \jmp^{\aval}_i(\tau_j)}$\\
			\hline
			$\jumps^{\gamma}(\tau_j)$ & $\sum_{i=1}^k \mathds{1}\set{\jmp^{\gamma}_i(\tau_j) < \infty}$\\
			\hline
			$\jumps^{\rho}(\tau_j)$ & $\sum_{i=1}^k \mathds{1}\set{\jmp^{\rho}_i(\tau_j) < \infty}$\\
			\hline
			$\jumps^{\aval}(\tau_j)$ & $\sum_{i=1}^k \mathds{1}\set{\jmp^{\aval}_i(\tau_j) < \infty}$\\
			\hline
			$\jumps(\tau_j)$ & $\sum_{i=1}^k \mathds{1}\set{\jmp_i(\tau_j) < \infty}$\\
			\hline
		\end{tabular}
	\end{center}
\end{table}


\subsection{Proving \texorpdfstring{\cref{lemma:all-Bs-are-1}}{the section's lemma} Using \texorpdfstring{\cref{lemma:bad_events:main-lemma}}{the main technical lemma of this section}}\label{sec:bad_events:proving-lemma}

\remove{
\Bnote{This should be the start of section 7, where a restatement of
	\cref{lemma:all-Bs-are-1} should appear. You can also look at the restatement
	environment I use in \cref{sec:ext:definitions}} 

\Bnote{In the beginning of this
	section you say that the asymptotic is w.r.t. $n$. Here it is not the case as
	far as I can see. Am I right? This issue is throughout this section}.

\Bnote{I
	also think that this is the place for a high level explanation of what about
	to happen. Saying that $W$ is a sufficiently-high probability event over the
	product transcript. The bits are representing typical behavior of the product
	transcript and if they are zero under $W$, then $W$ cannot happen with high
	probability} 
}


In this section we prove \cref{lemma:all-Bs-are-1} by showing that if $k$ and $\Unf[W]$ are large enough, then $\wIdl_{B^{m+2}}(1^{m+2})$ must be close to $1$. Recall that by the definition of $\wIdl$ (defined in
\cref{def:P-hat}), each bit $B_j$ equals to the product
$B_j^{\hist}\cdot B_j^{\indx} \cdot B_j^{\cur}$. In the following, we
extend the distribution of $\wIdl$ by separating the bits $B^{\hist}_j$
into two new bits $B^{\largeset}_j$ and $B^{\expcur}_j$ such that
$\wIdl_{B^{\hist}_j | B^{\largeset}_j, B^{\expcur}_j} = B^{\largeset}_j
\cdot B^{\expcur}_j$. We do so by defining
$\wIdl_{B^{\largeset}_0} = \mathds{1}\set{\size{\cD} \geq k\cdot
	2^{\ell-1}}$ and
$\wIdl_{B^{\expcur}_0} = \mathds{1}\set{\eex{\Idl_{Z^k X_{1}^k}}{\wIdl_{B_0^{\cur} | Z^k X_{1}^k}(0)} \leq \frac{m}{k^2}}$, and
for $j \in [m+1]$ we define
$\wIdl_{B^{\largeset}_j | Z^k X_{<j}^k} = \mathds{1}\set{\size{\GSet_{Z^k
			X_{<j}^k}} \geq \frac{k}{10}}$ and
$\wIdl_{B^{\expcur}_j | Z^k X_{<j}^k} = \mathds{1}\set{\eex{\Idl_{X^k_j | Z^k
			X^k_{<j}}}{\wIdl_{B_j^{\cur}|Z^k X_{\leq j}^k}(0)} \leq
	\frac{m}{k^2}}$.

\remove{
\Bnote{Instead of this paragraph I think that three (or four) claims should
	appear that claim: if these bits (either hist, index etc.) are 0 with high
	probability then $\Pr[W]$ is low. It seems that these are the corollaries from
	next few sections. After these claims should be the proof of
	\cref{lemma:all-Bs-are-1} that is now in
	\cref{sec:bad_events:all_together}. After this proof should come
	\cref{claim:bad_events:\jmp_i} and any other claim you relay on for proving
	the claims about the bits. Here is where the definition of this $\jmp$ will
	also be since it is needed for \cref{claim:bad_events:\jmp_i}}
}

In order to prove \cref{lemma:all-Bs-are-1}, we handle each type of bit separately. In \cref{sec:bad_events:large_set_bits} we handle the $B_j^{\largeset}$ bits, in \cref{sec:bad_events:index_bits} we hande the $B_j^{\indx}$ bits, and in \cref{sec:bad_events:cur_round_bits} we handle the $B_j^{\cur}$ and $B_j^{\expcur}$ bits. Finally, in \cref{sec:bad_events:all_together} we collect all parts and deduce the proof of \cref{lemma:all-Bs-are-1}.

\subsubsection{The Large-Set Bits}\label{sec:bad_events:large_set_bits}

Before handling the ``large-set'' bits, we first prove the following simple claim which state that the set of active verifiers $\ISet_{X^{(m+1) \times k}}$ is large.

\begin{claim}\label{claim:bad_events:ISet}
	There exists a universal constant $\lambda > 0$ such that for any $q \in (0,1)$ the following holds: If $\Idl\left[\size{\ISet_{X^{(m+1) \times k}}} \leq \frac{k}9\right] \geq q$,  then $\Unf[W] \leq \frac1{q}\cdot e^{-\zfrac{k}{\lambda}}$.
\end{claim}
\begin{proof}
	Assume $\Idl\left[\size{\ISet_{X^{(m+1) \times k}}} \leq \frac{k}9\right] \geq q$ for some $q \in (0,1)$.
	Observe that the distribution of $\size{\ISet_{X^{(m+1) \times k}}}$ when $X^{(m+1) \times k}$ is drawn from  $\Unf_{X^{(m+1) \times k}}$ is exactly $\Bin(k,(1-\frac1{m})^{m+1})$. Since $(1-\frac1{m})^{m+1} \geq \frac18$ for $m \geq 2$, Hoeffding's inequality (\cref{fact:prelim:indep_concent:hoeffding}) yields that
	\begin{align*}
		\Unf\left[\size{\ISet_{X^{(m+1) \times k}}} \leq  \frac{k}9\right]
		&\leq \pr{\Bin(k,\zfrac18) \leq \zfrac{k}9}\\
		&\leq e^{-\zfrac{k}{\lambda}},
	\end{align*}
	for some universal constant $\lambda > 0$, and we conclude that
	\begin{align*}
		\Unf[W]
		\leq \frac{\Unf\left[\size{\ISet_{X^{(m+1) \times k}}} \leq \frac{k}9\right]}{\Idl\left[\size{\ISet_{X^{(m+1) \times k}}} \leq \frac{k}9\right]}
		\leq \frac1{q}\cdot e^{-\zfrac{k}{\lambda}}
	\end{align*}
	as required.
\end{proof}

In addition, we prove that if $\Unf[W]$ is high enough and if $k$ is large enough, then the probability (over $\Idl$) that $\size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}$ is high.

\begin{claim}\label{claim:bad_events:GSet-bound}
	For any constant $\lambda > 0$, there exists constants $\lambda',\lambda'' > 0$ such that the following holds: If
	$\Idl[\size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}] \leq 1 -  \zfrac{\eps}{\lambda}$ and $k \geq \zfrac{\lambda'}{\eps}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'' \cdot m}}$.
\end{claim}
\begin{proof}
	Assume that $\Idl[\size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}] \leq 1 -  \zfrac{\eps}{\lambda}$ for some constant $\lambda > 0$.\remove{In the following we assume \wlg that $\size{\GSet} \geq 0.999 k$ since otherwise, the proof follows by \cref{lemma:bad_events:main-lemma}(\ref{item:bad_events:main-claim:G}).} Note that by definition, for any fixed $Z^k X^{(m+1)\times k}$ it holds that
	\begin{align}
		\size{\GSet_{Z^k X^{(m+1)\times k}}}
		&\geq \size{\ISet_{X^{(m+1) \times k}}} - (k - \size{\GSet}) - \jumps(Z^k X^{(m+1)\times k})
	\end{align}
	By assumption, one of the following items must hold: 
	\begin{enumerate}
		\item $\size{\GSet} \leq 0.999 k$, or\label{item:bad_events:GSet-bound:G}
		\item $\Idl\left[\size{\ISet_{Z^k X^{(m+1)\times k}}} \leq \frac{k}{9}\right] \geq \zfrac{\eps}{2 \lambda}$, or\label{item:bad_events:GSet-bound:I}
		\item $\Idl\left[\jumps(Z^k X^{(m+1)\times k}) \geq 0.001 k\right] \geq \zfrac{\eps}{2 \lambda}$.\label{item:bad_events:GSet-bound:jumps}
	\end{enumerate}
	If \cref{item:bad_events:GSet-bound:G} holds, then we deduce from  \cref{lemma:bad_events:main-lemma}(\ref{item:bad_events:main-claim:D}) that $\Unf[W] \leq (1-\eps)^{\frac{k}{c \cdot m}}$, where $c$ is the constant $\lambda' = \lambda'(1000)$ of  \cref{lemma:bad_events:main-lemma} (note that $\size{\cD} \leq \size{\GSet}\cdot 2^{\ell}$). 
	If \cref{item:bad_events:GSet-bound:I} holds, then we deduce from \cref{claim:bad_events:ISet} that $\Unf[W] \leq \frac{2\lambda}{\eps} \cdot e^{-\zfrac{k}{c'}} \leq (1-\eps)^{\frac{k}{2c'}}$, where $c'$ is the universal constant $\lambda'$ of \cref{claim:bad_events:ISet}, and the second inequality holds by choosing the claim's constant $\lambda'$ to be large enough such that  $k > \zfrac{\lambda'}{\eps}$ implies it. If \cref{item:bad_events:GSet-bound:jumps} holds, then in particular it holds that
	\begin{align*}
		\eex{\Idl}{\jumps(Z^k X^{(m+1)\times k})} \geq \frac{\eps k}{2000 \lambda}
	\end{align*}
	Hence, we deduce from \cref{lemma:bad_events:main-lemma}(\ref{item:bad_events:main-claim:jumps}) that $\Unf[W] \leq (1-\eps)^{\frac{k}{c'' \cdot m}}$ where $c''$ is the constant $\lambda' = \lambda'(2000 \lambda)$ of \cref{lemma:bad_events:main-lemma}. By setting the claim's constant $\lambda'' = \max\set{c,2c',c''}$, the proof follows.
	
\end{proof}

As a corollary of \cref{lemma:bad_events:main-lemma,claim:bad_events:GSet-bound}, it holds that if $k$ and $\Unf[W]$ are large enough, then the probability of failure (over $\wIdl$) in the ``large\_set'' bits is low.

\begin{corollary}\label{corollary:bad_events:B_gset}
	For any constant $\lambda > 0$, there exists constants $\lambda',\lambda'' > 0$ such that the following holds: If
	$\wIdl_{B^{\largeset}_0,\ldots,B^{\largeset}_{m+1}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ and $k \geq \zfrac{\lambda'}{\eps}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'' \cdot m}}$.
\end{corollary}

\begin{proof}
	Assume that $\wIdl_{B^{\largeset}_0,\ldots,B^{\largeset}_{m+1}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ for some constant $\lambda > 0$.
	If $\wIdl_{B^{\largeset}_0}(1) = 0$, then $\size{\cD} \leq k \cdot 2^{\ell - 1}$ and the proof follows by \cref{lemma:bad_events:main-lemma}(\ref{item:bad_events:main-claim:D}). Otherwise, $\wIdl_{B^{\largeset}_0}(1) = 1$ and therefore, $\wIdl_{B^{\largeset}_1,\ldots,B^{\largeset}_{m+1}}(1^{m+2}) \leq 1 -  \zfrac{\eps}{\lambda}$. Since  $\wIdl_{Z^k X^{(m+1) \times k}} \equiv \Idl$ and since $\wIdl_{B^{\largeset}_0,\ldots,B^{\largeset}_{m+1} | Z^k X^{(m+1) \times k}}(1^{m+2}) = \mathds{1}\set{\size{\GSet_{Z^k X^{m\times k}}} \geq \frac{k}{10}} \geq \mathds{1}\set{\size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}}$ (for any fixed $Z^k X^{(m+1)\times k}$), we deduce that $\Idl[\size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}] \leq 1 -  \zfrac{\eps}{\lambda}$ and the proof follows by \cref{claim:bad_events:GSet-bound}.	
\end{proof}

\subsubsection{The Index Bits}\label{sec:bad_events:index_bits}

In order to bound the probability of failure (over $\wIdl$) in the ``index'' bits, we make use of the following two claims. The proof of the first claim appears in \cref{corollary:bad_events:large-gammas-rest}.

\def\LargeGammasClaim{
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $ \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i} \cdot \mathds{1}\set{\gamma_{j,i} > 1}} \geq \zfrac{\eps k}{\lambda}$ for $\gamma_{j,i} = \gamma_{j,i}(Z^k X^{(m+1)\times k})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
}

\begin{claim}\label{claim:bad_events:large-gammas}
	\LargeGammasClaim
\end{claim}

\begin{claim}\label{claim:bad_events:1-and-gamma}
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} (1 + \gamma_{j,i})\cdot \mathds{1}\set{\jmp_i =j}} \geq \zfrac{\eps k}{\lambda}$ for $\gamma_{j,i} = \gamma_{j,i}(Z^k X^k_{<j})$ and $\jmp_i = \jmp_i(Z^k X^{(m+1)\times k})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{claim}
\begin{proof}
	Observe that
	\begin{align*}
		\lefteqn{\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} (1 + \gamma_{j,i})\cdot \mathds{1}\set{\jmp_i =j}}}\\
		&= \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} (1 + \gamma_{j,i})\cdot \mathds{1}\set{\jmp_i =j} \cdot \left(\mathds{1}\set{\gamma_{j,i} \leq 1} + \mathds{1}\set{\gamma_{j,i} > 1}\right)}\\
		&\leq 2 \cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \mathds{1}\set{\jmp_i =j}} + 2 \cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i} \cdot \mathds{1}\set{\gamma_{j,i} > 1}}\\
		&= 2 \cdot \eex{\Idl}{\jumps(Z^k X^{(m+1)\times k})} + 2 \cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i} \cdot \mathds{1}\set{\gamma_{j,i} > 1}},
	\end{align*}
	By assumption, at least one of the following items must holds:
	\begin{enumerate}
		\item $\eex{\Idl}{\jumps(Z^k X^{(m+1)\times k})} \geq \frac{\eps}{4 \lambda}$, or\label{item:bad_events:1-and-gamma:jumps}
		\item $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i} \cdot \mathds{1}\set{\gamma_{j,i} > 1}} \geq \frac{\eps}{4 \lambda}$.\label{item:bad_events:1-and-gamma:gamma}
	\end{enumerate}
	If \cref{item:bad_events:1-and-gamma:jumps} holds, then \cref{lemma:bad_events:main-lemma}(\ref{item:bad_events:main-claim:jumps}) implies that $\Unf[W] \leq (1-\eps)^{\frac{k}{c \cdot m}}$, where $c > 0$ is the constant $\lambda' = \lambda'(4 \lambda) > 0$ of \cref{lemma:bad_events:main-lemma}. If \cref{item:bad_events:1-and-gamma:gamma} holds then \cref{claim:bad_events:large-gammas} implies that $\Unf[W] \leq (1-\eps)^{\frac{k}{c' \cdot m}}$, where $c' > 0$ is the constant $\lambda' = \lambda'(4 \lambda) > 0$ of \cref{claim:bad_events:large-gammas}. Hence, the proof follows by setting $\lambda' = \max\set{c,c'}$.
\end{proof}


As a corollary of \cref{claim:bad_events:1-and-gamma}, if $k$ and $\Unf[W]$ are large enough, then the probability of failure (over $\wIdl$) in the ``index'' bits is low.

\begin{corollary}\label{corollary:bad_events:Bindx}
	For any constant $\lambda > 0$, there exists constants $\lambda',\lambda'' > 0$ such that the following holds: 
	If $\wIdl_{B^{\indx}_0,\ldots,B^{\indx}_{m+1}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ and $k \geq \zfrac{\lambda'}{\eps}$, then $\Unf[W] \leq (1-\eps)^{\lambda'' \cdot \zfrac{k}{m}}$.
\end{corollary}

\begin{proof}
	Assume that $\wIdl_{B^{\indx}_0,\ldots,B^{\indx}_{m+1}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ for some constant $\lambda > 0$. If $\wIdl_{B^{\indx}_0}(0) \geq \frac{\eps}{2\lambda}$, then $\size{\cD} \leq (1 - \frac{\eps}{2\lambda}) \cdot k \cdot 2^{\ell}$ and by \cref{lemma:bad_events:main-lemma}(\ref{item:bad_events:main-claim:D}) we deduce that $\Unf[W] \leq (1-\eps)^{\frac{k}{c \cdot m}}$, where $c > 0$ is the constant $\lambda' = \lambda'(2 \lambda) > 0$ of \cref{lemma:bad_events:main-lemma}. Otherwise, it holds that $\wIdl_{B^{\indx}_1,\ldots,B^{\indx}_{m+1}}(1^{m+2}) < 1 - \frac{\eps}{2\lambda}$. Observe that for any fixing of $Z^k X^{(m+1)\times k}$ with $\size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}$ and for any $j \in [m+1]$, it holds that
	\begin{align}\label{eq:bad_events:Bindx-round_j}
		\wIdl_{B^{indx}_j | Z^k X^k_{<j}}(0)
		&= \ppr{i \sim \Rll_{I|Z^k X^k_{<j},I\in \GSet_{j-1}}}{i \notin \GSet_{j}}\nonumber\\
		&= \frac{\sum_{i \in \GSet_{j-1} \setminus \GSet_{j}}\aval_{j,i}}{\sum_{i' \in \GSet_{j-1}} \aval_{j,i'}}\nonumber\\
		&= \frac{\sum_{i \in \GSet_{j-1} \setminus \GSet_{j}}\aval_{j-1,i}\cdot \frac{\Idl_{X_{j,i} | Z^k X^k_{<j'}}(1)}{\Idl_{X_{j,i} | Z^k X^k_{<j-1}}(1)}}{\sum_{i' \in \GSet_{j-1}} \aval_{j,i'}}\nonumber\\
		&\leq \frac{\sum_{i \in \GSet_{j-1} \setminus \GSet_{j}} 10 \cdot \frac{\Idl_{X_{j,i} | Z^k X^k_{<j'}}(1)}{\frac{1-0.1}m(1-\frac1{m})}}{0.01 \cdot \size{\GSet_{j}}}\nonumber\\
		&\leq 25000\cdot \frac{m}{k}\cdot \sum_{i \in \GSet_{j-1} \setminus \GSet_{j}} \Idl_{X_{j,i} | Z^k X^k_{<j'}}(1)\nonumber\\
		&= 25000\cdot \frac{1}{k}\cdot \sum_{i=1}^k (1 + \gamma_{j,i})\cdot \mathds{1}\set{\jmp_i = j},
	\end{align}
	where we let $\GSet_{j-1} = \GSet_{Z^k X^k_{<j-1}}$ and $\GSet_{j} = \GSet_{Z^k X^k_{<j}}$.
	The second equality in (\ref{eq:bad_events:Bindx-round_j}) holds by \cref{claim:PR_Thm:I_dist}, the first inequality holds since $i \in \GSet_{j-1} \implies a_{j-1,i} \in [0.01,10], \size{\rho_{j-1,i}} \leq 0.1$ and since $\sum_{i' \in \GSet_{j-1}} \aval_{j,i'} \geq \sum_{i' \in \GSet_{j}} \aval_{j,i'} \geq 0.01\cdot \size{\GSet_{j}}$, and the last inequality holds since $\size{\GSet_{j}} \geq \size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}$ and since $m \geq 2$. Therefore, by assumption we deduce that
	\begin{align*}
		\frac{\eps}{2\lambda}
		&\leq \wIdl_{B^{\indx}_1,\ldots,B^{\indx}_{m+1}}[\exists j\in[m+1]\text{ s.t. }B^{\indx}_j = 0]\\
		&\leq \sum_{j=1}^{m+1} \wIdl_{B^{\indx}_j}(0)\\
		&= \eex{\Idl}{\sum_{j=1}^{m+1} \wIdl_{B^{\indx}_j | Z^k X^k_{<j}}(0)}\\
		&\leq \eex{\Idl}{\sum_{j=1}^{m+1} \wIdl_{B^{\indx}_j | Z^k X^k_{<j}}(0) \mid \size{\GSet_{Z^k X^{(m+1)\times k}}} \geq \frac{k}{10}} + \Idl\left[\size{\GSet_{Z^k X^{(m+1)\times k}}\right] \geq \frac{k}{10}}\\
		&\leq 25000 \cdot \frac{1}{k}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} (1 + \gamma_{j,i})\cdot \mathds{1}\set{\jmp_i = j}} + \Idl\left[\size{\GSet_{Z^k X^{(m+1)\times k}}\right] \geq \frac{k}{10}},
	\end{align*}
	where the last inequality holds by \cref{eq:bad_events:Bindx-round_j}.
	Hence, one of the above two item must hold:
	\begin{enumerate}
		\item $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} (1 + \gamma_{j,i})\cdot \mathds{1}\set{\jmp_i = j}} \geq \frac{\eps k}{10^5 \cdot \lambda}$, or\label{item:bad_events:Bindx:1-plus-gamma}
		\item $\Idl\left[\size{\GSet_{Z^k X^{(m+1)\times k}}\right] \geq \frac{k}{10}} \geq \frac{\eps}{4\lambda}$.\label{item:bad_events:Bindx:GSet}
	\end{enumerate}
	If \cref{item:bad_events:Bindx:1-plus-gamma} holds, then \cref{claim:bad_events:1-and-gamma} implies that $\Unf[W] \leq (1-\eps)^{\frac{\eps k}{c' \cdot m}}$ where $c'$ is the constant $\lambda' = \lambda'(10^5 \cdot \lambda)$ of \cref{claim:bad_events:1-and-gamma}. If \cref{item:bad_events:Bindx:GSet} holds, then by setting the constant $\lambda'$ of the claim to the constant $\lambda' = \lambda'(4\lambda)$ of \cref{claim:bad_events:GSet-bound}, we obtain that \cref{claim:bad_events:GSet-bound} implies that $\Unf[W] \leq (1-\eps)^{\frac{\eps k}{c'' \cdot m}}$ where $c''$ is the constant $\lambda''= \lambda''(4\lambda)$ of  \cref{claim:bad_events:GSet-bound}. The proof then follows by setting the constant $\lambda''$ of the corollary to $\lambda'' = \max\set{c,c',c''}$.
\end{proof}


\subsubsection{The Current-Round Bits}\label{sec:bad_events:cur_round_bits}

In this section we handle the $B_j^{\cur}$ and $B_j^{\expcur}$ bits. Assuming that $\Unf[W]$ is large enough, the
following claim states that if $B_j^{\largeset} = 1$ (\ie the set of``good'' columns
$\GSet_{Z^k X^k_{<j}}$ is large) then $B_j^{\expcur} = 1$ (\ie
the probability that $\size{\delta_j} > 0.5$ is small).

\begin{claim}\label{claim:bad_events:B_expcur}
	There exists two constants $\lambda,\lambda' > 0$ such that the following holds: If $k \geq \lambda \cdot m^2$ and $\exists j \in (m+1)$ such that $\wIdl_{B_j^{\largeset}, B_j^{\expcur}}(1,0) > 0$,
	then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{claim}
\begin{proof}
	We separately handle two cases: $j=0$ and $j \in [m+1]$.
	
	\textbf{The case $j=0$:}
	In this case, it holds that $\size{\cD} \geq k \cdot 2^{\ell-1}$ (in particular, $\size{\GSet} \geq \frac{k}2$), and that
	\begin{align}\label{eq:bad_events:next_bit_0:zero_rnd_assum}
		\Idl_{Z^k X^k_{1}}\left[\size{\ddelta_0(Z^k X^k_{1})} > 0.5\right] > \frac{m}{k^2}.
	\end{align}
	and recall that
	\begin{align*}
		\ddelta_0(z^k x_1^k) = \zfrac{\left(\sum_{i \in 1_{x_1^k}} \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)}\right)}{\left(\zfrac{\size{\cD}}{2^{\ell}}\right)} - 1
	\end{align*}
	In the following, we define
	\begin{enumerate}
		\item $\ddelta^X_0(x_1^k ; z^k) = \zfrac{\left(\sum_{i \in 1_{x_1^k}} \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)}\right)}{\left(\sum_{i=1}^k \aval_{0,i}(z_i)\right)} - 1$,
		\item $\ddelta^Z_0(z^k) = \zfrac{\left(\sum_{i=1}^k \aval_{0,i}(z_i)\right)}{\left(\zfrac{\size{\cD}}{2^{\ell}}\right)} - 1 = \zfrac{\left(\sum_{i=1}^k \frac{\mathds{1}\set{(i,z) \in \cD}}{\Idl_{Z_i | X_{1,i}=1}(z_i)}\right)}{\size{\cD}} - 1$.
	\end{enumerate}
	and observe that
	\begin{align}\label{eq:bad_events:next_bit_0:zero_rnd_separation}
		\ddelta_0
		&= \zfrac{\left(\bigl(1 + \ddelta^X_0\bigr)\cdot \sum_{i=1}^k \aval_{0,i}\right)}{\left(\zfrac{\size{\cD}}{2^{\ell}}\right)} - 1\nonumber\\
		&= \zfrac{\left(\bigl(1 + \ddelta^X_0\bigr)\cdot \bigl(1 + \ddelta^Z_0\bigr) \cdot \zfrac{\size{\cD}}{2^{\ell}} \right)}{\left(\zfrac{\size{\cD}}{2^{\ell}}\right)} - 1\nonumber\\
		&= \ddelta^X_0 + \ddelta^Z_0 + \ddelta^X_0 \cdot \ddelta^Z_0
	\end{align}
	Therefore, by \cref{eq:bad_events:next_bit_0:zero_rnd_assum,eq:bad_events:next_bit_0:zero_rnd_separation}, one of the following must holds
	\begin{enumerate}
		\item $\Idl_{Z^k X^k_{1}}\left[\size{\ddelta^X_0(X^k_{1} ; Z^k)} > 0.2\right] > \frac{m}{2k^2}$, or
		\item $\Idl_{Z^k}\left[\size{\ddelta^Z_0(Z^k)} > 0.2\right] > \frac{m}{2k^2}$
	\end{enumerate}
	
	Note that the sum $\sum_{i=1}^k \frac{\mathds{1}\set{(i,z) \in \cD}}{\Idl_{Z_i | X_{1,i}=1}(z_i)}$ when $z^k$ is drawn from $\Unf_{Z^k}$ is a sum of $k$ independent random variable, where
	\begin{align}\label{eq:bad_events:Bcur_0:Delta_Z_exp}
		\eex{z^k \sim \Unf_{Z^k}}{\sum_{i=1}^k \frac{\mathds{1}\set{(i,z) \in \cD}}{\Idl_{Z_i | X_{1,i}=1}(z_i)}}
		&= \sum_{z \in \zo^{\ell}} \sum_{i=1}^k 2^{-\ell}\cdot \frac{\mathds{1}\set{(i,z) \in \cD}}{\Idl_{Z_i | X_{1,i}=1}(z_i)}\nonumber\\
		&\in \frac1{1 \pm 0.1} \cdot \sum_{z \in \zo^{\ell}} \sum_{i=1}^k \mathds{1}\set{(i,z) \in \cD}\nonumber\\
		&\subseteq (0.9,1.15) \cdot \size{\cD}
	\end{align}
	
	and the \ith variable is bounded in the interval $[0,\frac{1}{1-0.1} \cdot 2^{\ell}] \subseteq [0,1.15 \cdot 2^{\ell}]$. Therefore,
	\begin{align}\label{eq:bad_events:Bcur_0:Delta_Z}
		\lefteqn{\ppr{z^k \sim \Unf_{Z^k}}{\size{\ddelta^Z_0(z^k)} > 0.2}}\nonumber\\
		&= \ppr{z^k \sim \Unf_{Z^k}}{\size{\sum_{i=1}^k \frac{\mathds{1}\set{(i,z) \in \cD}}{\Idl_{Z_i | X_{1,i}=1}(z_i)} - \size{\cD}} > 0.2\cdot \size{\cD}}\nonumber\\
		&\leq \ppr{z^k \sim \Unf_{Z^k}}{\size{\sum_{i=1}^k \frac{\mathds{1}\set{(i,z) \in \cD}}{\Idl_{Z_i | X_{1,i}=1}(z_i)} - \eex{z^k \sim \Unf_{Z^k}}{\sum_{i=1}^k \frac{\mathds{1}\set{(i,z) \in \cD}}{\Idl_{Z_i | X_{1,i}=1}(z_i)}}} > 0.05 \cdot \size{\cD}}\nonumber\\
		&\leq 2\cdot \exp\paren{-\frac{2 \cdot (0.05 \cdot \size{\cD})^2}{k \cdot (1.15 \cdot 2^{\ell})^2}}\nonumber\\
		&\leq 2\cdot \exp\paren{-\frac{k}{2\cdot 10^3 m}}
	\end{align}
	where the first inequality holds by \cref{eq:bad_events:Bcur_0:Delta_Z_exp}, the second one by \cref{fact:prelim:indep_concent:hoeffding} (Hoeffding's inequality) and the last one holds since $\size{\cD} \geq k\cdot 2^{\ell -1}$.
	
	In the following, fix $z^k$ with $\size{\ddelta^Z_0(z^k)} \leq 0.2 \implies 
	\zfrac{\left(\sum_{i=1}^k \aval_{0,i}(z_i)\right)}{\left(\zfrac{k \cdot 2^{\ell - 1}}{2^{\ell}}\right)} - 1 \geq -0.2 \implies \sum_{i=1}^k \aval_{0,i}(z_i) \geq 0.4 k$. Note that the sum $\sum_{i \in 1_{x_1^k}} \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)}$ when $x_1^k$ is drawn from $\Unf_{X^k_1}$ is a sum of $k$ independent random variables, where the \ith variable (which corresponds to $\mathds{1}\set{x_1^k = 1} \cdot \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)}$) is distributed according to $b_i \cdot \Bern(\zfrac1{m})$ for $b_i = \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)} \in \frac{\aval_{0,i}(z_i)}{(1 \pm 0.1)\cdot \zfrac{1}{m}} \subseteq (0.9,1.15)\cdot m\cdot  \aval_{0,i}(z_i)$. Therefore,
	\begin{align}\label{eq:bad_events:Bcur_0:Delta_X_exp}
		\eex{x^k_1 \sim \Unf_{X^k_1}}{\sum_{i \in 1_{x_1^k}} \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)}} \in \frac{1}{1 \pm 0.1} \cdot \sum_{i=1}^k \aval_{0,i}(z_i) \subseteq (0.9,1.15)\cdot \sum_{i=1}^k \aval_{0,i}(z_i)
	\end{align}
	and we obtain that
	\begin{align}\label{eq:bad_events:Bcur_0:Delta_X}
		\lefteqn{\ppr{x^k_{1} \sim \Unf_{X^k_{1}}}{\size{\ddelta^X_0(x^k_{1} ; z^k)} > 0.2}}\nonumber\\
		&= \ppr{x^k_{1} \sim \Unf_{X^k_{1}}}{\size{\sum_{i \in 1_{x_1^k}} \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)} - \sum_{i=1}^k \aval_{0,i}(z_i)} > 0.2 \cdot \sum_{i=1}^k \aval_{0,i}(z_i)}\nonumber\\
		&\leq \ppr{x^k_{1} \sim \Unf_{X^k_{1}}}{\size{\sum_{i \in 1_{x_1^k}} \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)} - \eex{x^k_1 \sim \Unf_{X^k_1}}{\sum_{i \in 1_{x_1^k}} \frac{\aval_{0,i}(z_i)}{\Idl_{X_{1,i}}(1)}}} > 0.05 \cdot \sum_{i=1}^k \aval_{0,i}(z_i)}\nonumber\\
		&\leq 2 \exp\paren{-\frac{(0.05 \cdot \sum_{i=1}^k \aval_{0,i}(z_i))^2}{2(\sum_{i=1}^k \zfrac{b_i^2}m + \max\set{b_i} \cdot \zfrac{0.05 \cdot \sum_{i=1}^k \aval_{0,i}(z_i)}3)}}\nonumber\\
		&\leq 2 \exp\paren{-\frac{k}{10^4 m}}
	\end{align}
	where the first inequality holds by \cref{eq:bad_events:Bcur_0:Delta_X_exp}, the second one holds by \cref{fact:prelim:indep_concent:variance} and the third one holds since $\max\set{b_i} \leq 2m$ and $\sum_{i=1}^k \aval_{0,i}(z_i) \geq 0.4k$.
	
	Using \cref{eq:bad_events:Bcur_0:Delta_Z,eq:bad_events:Bcur_0:Delta_X}, we conclude that
	
	\begin{align*}
		\Unf_{Z^k X^k_1}\left[\size{\ddelta_0(Z^k X^k_1)} > 0.5\right]
		&\leq \Unf_{Z^k}\left[\size{\ddelta^Z_0(Z^k)} > 0.2\right] + \Unf_{Z^k X^k_1 | \size{\ddelta^Z_0(Z^k)} \leq 0.2}\left[\size{\ddelta^X_0(X^k_1;Z^k)} > 0.2\right]\\
		&\leq 4 \cdot \exp\paren{-\frac{k}{10^4 m}},
	\end{align*}
	\begin{align*}
		\implies \Unf[W] \leq \frac{\Unf_{Z^k X^k_1}\left[\size{\ddelta_0(Z^k X^k_1)} > 0.5\right]}{\Idl_{Z^k X^k_1}\left[\size{\ddelta_0(Z^k X^k_1)} > 0.5\right]} \leq \frac{4 \cdot \exp\paren{-\frac{k}{10^4 m}}}{\zfrac{m}{k^2}} \leq (1-\eps)^{\frac{k}{2\cdot 10^4 m}},
	\end{align*}
	where the last inequality holds by choosing the constant $\lambda'$ of the claim to be large enough such that $k \geq \lambda' \cdot m^2$ implies it.
	
	\textbf{The case $j \in [m+1]$:} In this case, it holds that
	\begin{align}\label{eq:bad_events:next_bit_0:2}
		\Idl_{Z^k X^k_{<j}}\left[\size{\GSet_{Z^k X_{<j}^k}} \geq \zfrac{k}{10} \land  \Idl_{X^k_{j+1} | Z^k X^k_{<j}}\left[\size{\ddelta_j(X^k_{j+1};Z^k X^k_{<j})} > 0.5\right] > \frac{m}{k^2}\right] >0
	\end{align}
	In particular, there exists $z^k x^k_{<j} \in \Supp(\Idl_{Z^k X^k_{<j}})$  that satisfy both conditions.
	In the following, fix such $z^k x^k_{<j}$.
	Recall that
	\begin{align*}
		\left(1 + \ddelta_j(x^k_{j+1}; z^k x^k_{<j})\right)\cdot \sum_{i \in \GSet_{z^k x^k_{<j}}} \aval_{j,i}
		= \sum_{i \in \GSet_{z^k x^k_{<j}} \bigcap 1_{x^k_{j+1}}} \frac{\aval_{j,i}}{\Idl_{X_{j+1,i} \mid Z^k X^k_{<j}}(1 | z^k x^k_{<j} )}
	\end{align*}
	where $\aval_{j,i} = \aval_{j,i}(z^k x^k_{<j})$ is according to \cref{fig:measurements}. Therefore, it holds that
	\begin{align}\label{eq:bad_events:B_next:pr_W_is_large_round_j}
		\lefteqn{\ppr{x^k_{j+1} \sim \Idl_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\size{\ddelta_j(x^k_{j+1};z^k x^k_{<j})} > \frac12}}\\
		&= \ppr{x^k_{j+1} \sim \Idl_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\sum_{i \in \cs \bigcap 1_{x^k_{j+1}}} \frac{\aval_i}{p_i}
			\notin (1 \pm 0.5) \sum_{i \in \cs} \aval_{i}}\nonumber\\
		&> \frac{m}{k^2}\nonumber
	\end{align}
	where we denote $\cs  = \GSet_{z^k x^k_{<j}}$ (recall that $\size{\cs} \geq \zfrac{k}{10}$), $\aval_i = \aval_{j,i}(z^k x^k_{<j}) \in [0.01,10]$ and $p_i = \Idl_{X_{j+1,i} \mid Z^k X^k_{<j}}(1 | z^k x^k_{<j}) \in (1 \pm 0.1)\cdot  \frac1{m}(1-\frac1{m})$. Observe that when taking $x^k_{j+1} \sim \Unf_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})$ (\ie without the conditioning on $W$), the term $\sum_{i \in \cs \bigcap 1_{x^k_{j+1}}} \frac{\aval_i}{p_i}$ is a sum of $\size{\cs} \geq \zfrac{k}{10}$ independent random variables, where the element that corresponds to $i \in \cs$ is distributed according to $b_i \cdot \Bern(\frac1{m}(1-\frac1{m}))$ for $b_i = \frac{\aval_i}{p_i} \in \frac1{1 \pm 0.1} \cdot \frac{\aval_i}{\frac1{m}(1-\frac1{m})}$. Therefore,
	\begin{align}\label{eq:bad_events:B_next:exp_round_j}
		\eex{x^k_{j+1} \sim \Unf_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\sum_{i \in \cs \bigcap 1_{x^k_{j+1}}} \frac{\aval_i}{p_i}} \in \frac1{1 \pm 0.1} \cdot \sum_{i \in \cs} \aval_i \subseteq (0.9, 1.15) \cdot \sum_{i \in \cs} \aval_i
	\end{align}
	
	and it holds that
	\begin{align}\label{eq:bad_events:B_next:pr_product_is_small_round_j}
		\lefteqn{\ppr{x^k_{j+1} \sim \Unf_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\size{\ddelta_j(x^k_{j+1};z^k x^k_{<j})} > 0.5}}\\
		&= \ppr{x^k_{j+1} \sim \Unf_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\size{\sum_{i \in \cs \bigcap 1_{x^k_{j+1}}} \frac{\aval_i}{p_i}} \notin (1 \pm 0.5) \cdot \sum_{i \in \cs} \aval_{i}}\nonumber\\
		&\leq \ppr{x^k_{j+1} \sim \Unf_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\size{\sum_{i \in \cs \bigcap 1_{x^k_{j+1}}} \frac{\aval_i}{p_i} - \eex{x^k_{j+1} \sim \Unf_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\sum_{i \in \cs \bigcap 1_{x^k_{j+1}}} \frac{\aval_i}{p_i}}} > 0.35 \cdot \sum_{i \in \cs} \aval_{i}}\nonumber\\
		&\leq 2\exp\paren{-\frac{0.35^2 \cdot (\sum_{i \in \cs} \aval_{i})^2}{2\left(\sum_{i \in \cs} \frac{\aval_i^2}{p_i^2}\cdot\frac1{m}(1-\frac1{m}) + 0.1 \cdot \max_{i \in \cs}\set{\frac{\aval_i}{p_i}} \cdot \sum_{i \in \cs} \aval_{i}\right)}}\nonumber\\
		&\leq 2\exp\paren{-\frac{0.35^2 \cdot (\sum_{i \in \cs} \aval_{i})^2}{2\left(300m\cdot \sum_{i \in \cs} \aval_i+30m \cdot \sum_{i \in \cs} \aval_{i}\right)}}\nonumber\\
		&\leq 2\exp\paren{-\frac{k}{6\cdot 10^6 m}},\nonumber
	\end{align}
	where the first inequality holds by \cref{eq:bad_events:B_next:exp_round_j}, the second one holds by \cref{fact:prelim:indep_concent:variance} and the last one holds since $\sum_{i \in \cs} \aval_{i} \geq 0.01 \cdot \size{S} \geq \zfrac{k}{10^3}$.
	
	Finally, by \cref{eq:bad_events:B_next:pr_W_is_large_round_j,eq:bad_events:B_next:pr_product_is_small_round_j}, we conclude that
	\begin{align*}
		\Unf[W] \leq \frac{\ppr{x^k_{j+1} \sim \Unf_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\size{\ddelta_j(x^k_{j+1};z^k x^k_{<j})} > 0.5}}{\ppr{x^k_{j+1} \sim \Idl_{X^k_{j+1} | Z^k X^k_{<j}}(\cdot | z^k x^k_{<j})}{\size{\ddelta_j(x^k_{j+1};z^k x^k_{<j})} > 0.5}} \leq \frac{2\exp\paren{-\frac{k}{6\cdot 10^6 m}}}{\zfrac{m}{k^2}} \leq (1-\eps)^{\frac{k}{10^7 m}},
	\end{align*}
	where the last inequality holds by choosing the constant $\lambda'$ of the claim to be large enough such that $k \geq \lambda' \cdot m^2$ implies it (recall that $\eps \in [0,\frac12]$).
\end{proof}

As a simple corollary of \cref{claim:bad_events:B_expcur}, if $k$ and $\Unf[W]$ are large enough, then the probability of failure (over $\wIdl$) in the ``expected current'' bits is low.

\begin{corollary}\label{corollary:bad_events:B_expcur}
	For any constant $\lambda > 0$ there exists constants $\lambda',\lambda'' > 0$ such that if $\wIdl_{B_0^{\expcur},\ldots,B_{m+1}^{\expcur}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ and $k \geq \lambda' \cdot \zfrac{m^2}{\eps}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'' \cdot m}}$.
\end{corollary}

\begin{proof}
	Assume that $\wIdl_{B_0^{\expcur},\ldots,B_{m+1}^{\expcur}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ for some constant $\lambda > 0$. By \cref{claim:bad_events:B_expcur}, we can focus on the case that $\wIdl_{B_0^{\expcur},\ldots,B_{m+1}^{\expcur} | B_0^{\largeset},\ldots,B_{m+1}^{\largeset}}(1^{m+2} | 1^{m+2}) = 1$. Note that
	\begin{align*}
		\wIdl_{B_0^{\largeset},\ldots,B_{m+1}^{\largeset}}(1^{m+2})
		\leq \frac{\wIdl_{B_0^{\expcur},\ldots,B_{m+1}^{\expcur}}(1^{m+2})}{\wIdl_{B_0^{\expcur},\ldots,B_{m+1}^{\expcur} | B_0^{\largeset},\ldots,B_{m+1}^{\largeset}}(1^{m+2} | 1^{m+2})}
		\leq 1 - \zfrac{\eps}{\lambda}
	\end{align*}
	Therefore, the proof follows by \cref{corollary:bad_events:B_gset}.
\end{proof}

The above yields that the probability of failure in the ``current'' bits is also low.

\begin{corollary}\label{corollary:bad_events:Bcur}
	For any constant $\lambda > 0$ there exists constants $\lambda',\lambda'' > 0$ such that if $\wIdl_{B_0^{\cur},\ldots,B_{m+1}^{\cur}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ and $k \geq \lambda' \cdot \zfrac{m^2}{\eps}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'' \cdot m}}$.
\end{corollary}
\begin{proof}
	Assume that $\wIdl_{B_0^{\cur},\ldots,B_{m+1}^{\cur}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ for some constant $\lambda > 0$. Note that
	\begin{align*}
		\wIdl_{B_0^{\expcur},\ldots,B_{m+1}^{\expcur}}(1^{m+2})
		&\leq \frac{\wIdl_{B_0^{\cur},\ldots,B_{m+1}^{\cur}}(1^{m+2})}{\wIdl_{B_0^{\cur},\ldots,B_{m+1}^{\cur} | B_0^{\expcur},\ldots,B_{m+1}^{\expcur}}(1^{m+2} | 1^{m+2})}\\
		&\leq \frac{1 - \zfrac{\eps}{\lambda}}{1 - (m+2)\cdot \frac{m}{k^2}}\\
		&\leq 1 - \frac{\eps}{2\lambda},
	\end{align*}
	where the last inequality holds by choosing the constant $\lambda'$ of the corollary to be large enough such that $k \geq \lambda' \cdot \zfrac{m^2}{\eps}$ implies it. 
	The proof then follows by \cref{corollary:bad_events:B_expcur}.
\end{proof}

As a corollary of \cref{corollary:bad_events:B_gset,corollary:bad_events:B_expcur}, if $k$ and $\Unf[W]$ are large enough, then the probability of failure (over $\wIdl$) in the ``history'' bits is low.

\begin{corollary}\label{corollary:bad_events:Bhist}
	For any constant $\lambda > 0$ there exists constants $\lambda',\lambda'' > 0$ such that if $\wIdl_{B_0^{\hist},\ldots,B_{m+1}^{\hist}}(1^{m+2}) \leq 1 - \zfrac{\eps}{\lambda}$ and $k \geq \lambda' \cdot \zfrac{m^2}{\eps}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'' \cdot m}}$.
\end{corollary}
\begin{proof}
	Immediately follows by \cref{corollary:bad_events:B_gset,corollary:bad_events:B_expcur} since $B^{\hist}_j = B^{\largeset}_j  \cdot B^{\expcur}_j$.
\end{proof}

\subsubsection{Putting It Together}\label{sec:bad_events:all_together}
The proof of \cref{lemma:all-Bs-are-1} is now trivially holds by the previous sections.
\begin{lemma}[Restatement of \cref{lemma:all-Bs-are-1}]
	\AllBsAreOneLemma
\end{lemma}
\begin{proof}
	Let $k,m,\ell,\eps,\cW,W,\Unf,\wIdl$ as in \cref{lemma:all-Bs-are-1} and assume that $\wIdl_{B^{m+2}}(1^{m+2}) < 1 -\zfrac{\eps}{\lambda}$ for some constant $\lambda > 0$. Since $B_j = B_j^{\cur} \cdot B_j^{\hist} \cdot B_j^{\indx}$, at least one of the following must hold:
	\begin{enumerate}
		\item $\wIdl_{B_0^{\cur},\ldots,B_{m+1}^{\cur}}(1^{m+2}) < 1 -\frac{\eps}{3\lambda}$, or
		\item $\wIdl_{B_0^{\hist},\ldots,B_{m+1}^{\hist}}(1^{m+2}) < 1 -\frac{\eps}{3\lambda}$, or
		\item $\wIdl_{B_0^{\indx},\ldots,B_{m+1}^{\indx}}(1^{m+2}) < 1 -\frac{\eps}{3\lambda}$.
	\end{enumerate}
	The proof then immediately follows by \cref{corollary:bad_events:Bcur,corollary:bad_events:Bhist,corollary:bad_events:Bindx}.
\end{proof}



\subsection{Proving \texorpdfstring{\cref{lemma:bad_events:main-lemma}}{the main technical lemma of this section}}\label{sec:bad_events:proving-main-lemma}

In this section, we prove \cref{lemma:bad_events:main-lemma}, restated for convenience below.

\BadEventMainLemma*
%\begin{lemma}[Restatement of \cref{lemma:bad_events:main-lemma}]
%	\BadEventMainLemma
%\end{lemma}

In the following, fix $k,m,\ell,\eps,\cW, W,\Unf,\Idl, \GSet, \cD$ as in \cref{lemma:bad_events:main-lemma}, and let $\jumps^{\gamma}, \jumps^{\rho}, \jumps^{\aval}$ the function from \cref{fig:bad_events:spec_rounds}.
The main components of \cref{lemma:bad_events:main-lemma}'s proof are divided into \cref{claim:bad_events:main-lemma-D-part,claim:bad_events:main-lemma-easy-jumps,claim:bad_events:main-lemma-hard-jumps}, proven separately in \cref{sec:bad_events:main-lemma-D-part,sec:bad_events:main-lemma-easy-jumps,sec:bad_events:main-lemma-hard-jumps}, respectively.

\def\MainLemmaDpart{
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $\size{\cD} \leq (1-\zfrac{\eps}{\lambda}) k\cdot 2^{\ell}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'\cdot m}}$.
}

\begin{claim}\label{claim:bad_events:main-lemma-D-part}
	\MainLemmaDpart
\end{claim}


\def\MainLemmaEasyJumps{
	For any constant $\lambda > 0$ there exists a constants $\lambda' > 0$ such that if $\eex{\Idl}{\jumps^{\nu}(Z^k X^{(m+1) \times k})} \geq \zfrac{\eps k}{\lambda}$ for some $\nu \in \set{\gamma,\rho}$,
	then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'\cdot m}}$.
}

\begin{claim}\label{claim:bad_events:main-lemma-easy-jumps}
	\MainLemmaEasyJumps
\end{claim}


\def\MainLemmaHardJumps{
	For any constant $\lambda > 0$, there exists a constant $\lambda' > 0$ such that if $\eex{\Idl}{\jumps^{\aval}(Z^k X^{(m+1) \times k})} \geq \zfrac{\eps k}{\lambda}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda'\cdot m}}$.
}

\begin{claim}\label{claim:bad_events:main-lemma-hard-jumps}
	\MainLemmaHardJumps
\end{claim}

The proof of \cref{lemma:bad_events:main-lemma} now trivially follows by \cref{claim:bad_events:main-lemma-D-part,claim:bad_events:main-lemma-easy-jumps,claim:bad_events:main-lemma-hard-jumps}.

\begin{proof}[Proof of \cref{lemma:bad_events:main-lemma}]
	Let $k,m,\ell,\eps,\cW, W,\Unf,\Idl$ as in \cref{lemma:bad_events:main-lemma} and assume that at least one of the following holds for some constant $\lambda > 0$:
	\begin{enumerate}
		\item $\size{\cD} \leq (1-\zfrac{\eps}{\lambda}) k\cdot 2^{\ell}$, or\label{item:bad_events:proof-main-claim:D}
		\item $\eex{\Idl}{\jumps(Z^k X^{(m+1) \times k})} \geq \zfrac{\eps k}{\lambda}$,\label{item:bad_events:proof-main-claim:jumps}
	\end{enumerate}
	If \cref{item:bad_events:proof-main-claim:D} holds then the proof follows by \cref{claim:bad_events:main-lemma-D-part}. Note that by definition of $\jumps$, it holds that $\jumps(\tau_j) \leq \sum_{\nu \in \set{\gamma, \rho, \aval}} \jumps^{\nu}(\tau_j)$ for any input $\tau_j$. Therefore, if \cref{item:bad_events:proof-main-claim:jumps} holds then there exists $\nu \in \set{\gamma,\rho,\aval}$ such that $\eex{\Idl}{\jumps^{\nu}(Z^k X^{(m+1) \times k})} \geq \frac{\eps k}{3\lambda}$. If the above holds for $\nu \in \set{\gamma,\rho}$, then the proof follows by \cref{claim:bad_events:main-lemma-easy-jumps}, and if it holds for $\nu = \aval$, then the proof follows by \cref{claim:bad_events:main-lemma-hard-jumps}.
\end{proof}

\subsubsection{Proving \texorpdfstring{\cref{claim:bad_events:main-lemma-D-part}}{the D part of main lemma}}\label{sec:bad_events:main-lemma-D-part}

Before proving \cref{claim:bad_events:main-lemma-D-part}, we start with a simple claim that connects the $\set{\rho_{0,i}}$'s measurements with $\Unf[W]$.

\begin{claim}\label{claim:bad_events:rho-zero}
	It holds that
	\begin{align*}
		\log{\frac1{\Unf[W]}} \geq \frac1{4m}\cdot \sum_{i=1}^k \min\set{\size{\rho_{0,i}}, \rho_{0,i}^2}
	\end{align*}
\end{claim}
\begin{proof}
	Compute
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \re{\Idl_{X^k_1}}{\Unf_{X^k_1}}
		= \re{\Idl_{X^k_1}}{\prod_{i=1}^{k} \Unf_{X_{1,i}}}\\
		&\geq \sum_{i=1}^k \re{\Idl_{X_{1,i}}}{\Unf_{X_{1,i}}}
		= \sum_{i=1}^k \re{\frac{1 + \rho_{0,i}}{m}}{\frac1m}\\
		&\geq \frac1{4m}\cdot \sum_{i=1}^k \min\set{\size{\rho_{0,i}}, \rho_{0,i}^2},
	\end{align*}
	where the first inequality holds by \cref{fact:kl-divergence:diver-cond-on-event}, the second one holds by \cref{fact:prelim:diver-properties} (the product case of chain rule) and the last one by \cref{fact:prelim:bernoulli-div-est}.
\end{proof}

As a corollary of \cref{claim:bad_events:rho-zero}, we obtain a lower bound on $\size{\GSet}$ in case $\Unf[W]$ is high enough.

\begin{corollary}\label{corollary:bad_events:rho-zero}
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $\size{\GSet} \leq (1 - \zfrac{\eps}{\lambda}) k$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{corollary}


\begin{proof}
	Assume that $\size{\GSet} \leq (1 - \zfrac{\eps}{\lambda}) k$ for some constant $\lambda > 0$. Then it holds that
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \frac1{4m}\cdot \sum_{i=1}^k \min\set{\size{\rho_{0,i}}, \rho_{0,i}^2}\\
		&\geq \frac1{4m}\cdot \sum_{i\in[k]\setminus \GSet} \min\set{\size{\rho_{0,i}}, \rho_{0,i}^2}\\
		&\geq \frac{0.01 \cdot (k - \size{\GSet})}{4m}
		\geq \frac{\eps k}{400\cdot m}
	\end{align*}
	\begin{align*}
		\implies \Unf[W] \leq e^{-\frac{\eps k}{400\cdot m}} \leq (1-\eps)^{\frac{\eps k}{800\cdot m}},
	\end{align*}
	where the first inequality holds by \cref{claim:bad_events:rho-zero} and the third one holds since $i \notin \GSet \implies \size{\rho_{0,i}} > 0.1$.
\end{proof}

The last claim we need in order to prove \cref{claim:bad_events:main-lemma-D-part} gives a lower bound on the average size of the sets $\set{\cZ_i}_{i \in [k]}$ (defined in \cref{fig:sets}) in case $\Unf[W]$ is high enough.


\begin{claim}\label{claim:bad_events:Z_i}
	For any constants $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if 
	$\eex{i \la \GSet}{\zfrac{\size{\cZ_i}}{2^{\ell}}} \leq 1 - \zfrac{\eps}{\lambda}$ then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{claim}

\begin{proof}
	Assume that $\eex{i \la \GSet}{\zfrac{\size{\cZ_i}}{2^{\ell}}} \leq 1 - \zfrac{\eps}{\lambda}$ for some constant $\lambda > 0$. If $\size{\GSet} < \zfrac{k}{2}$ then the proof immediately follows by \cref{corollary:bad_events:rho-zero}. Therefore, in the following we assume that $\size{\GSet} \geq \zfrac{k}{2}$. Observe that
	\begin{align}\label{eq:bad_events:Z_i:1}
		\log{\frac1{\Unf[W]}}
		&\geq \re{\Idl_{Z^k X^k_1}}{\Unf_{Z^k X^k_1}}
		= \re{\Idl_{Z^k X^k_1}}{\prod_{i=1}^k \Unf_{Z_i X_{1,i}}}\nonumber\\
		&\geq \sum_{i=1}^k \re{\Idl_{Z_i X_{1,i}}}{\Unf_{Z_i X_{1,i}}}
		\geq \sum_{i \in \GSet} \re{\Idl_{Z_i X_{1,i}}}{\Unf_{Z_i X_{1,i}}}\nonumber\\
		&\geq \sum_{i \in \GSet} \frac{1 + \rho_{0,i}}{m}\cdot \re{\Idl_{Z_i | X_{1,i}=1}}{\Unf_{Z_i}}\nonumber\\
		&\geq \frac{0.9}{m}\cdot \sum_{i \in \GSet} \re{\Idl_{Z_i | X_{1,i}=1}}{\Unf_{Z_i}}
	\end{align}
	where the first inequality holds by \cref{fact:kl-divergence:diver-cond-on-event} and the second one by \cref{fact:prelim:diver-properties} (the product case of chain rule).
	In the following, let $\bar{\cZ}_i^+ = \set{z \in \zo^{\ell} \colon \Idl_{Z_i | X_{1,i} = 1}(z) > (1 + 0.1)\cdot 2^{-\ell}}$ and $\bar{\cZ}_i^- = \set{z \in \zo^{\ell} \colon \Idl_{Z_i | X_{1,i} = 1}(z) < (1 - 0.1)\cdot 2^{-\ell}}$, and observe that $\bar{\cZ}_i^+ \bigcup \bar{\cZ}_i^- = \zo^{\ell} \setminus \cZ_i$. Therefore, by assumption it holds that 
	$\eex{i \la \GSet}{\zfrac{\size{\bar{\cZ}_i^+}}{2^{\ell}}} \geq \frac{\eps}{2\lambda}$ or $\eex{i \la \GSet}{\zfrac{\size{\bar{\cZ}_i^-}}{2^{\ell}}} \geq \frac{\eps}{2\lambda}$.
	If the first bound holds, then by \cref{eq:bad_events:Z_i:1} we obtain that
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \sum_{i \in \GSet} \frac{0.9}{m}\cdot \re{\Idl_{Z_i | X_{1,i}=1}(\bar{\cZ}_i^+)}{\Unf_{Z_i}(\bar{\cZ}_i^+)}\\
		&> \sum_{i \in \GSet} \frac{0.9}{m}\cdot \re{(1 + 0.1)\cdot \zfrac{\size{\bar{\cZ}^+_i}}{2^{\ell}}}{\zfrac{\size{\bar{\cZ}^+_i}}{2^{\ell}}}\\
		&\geq \frac{0.9 \cdot 0.1^2}{4m}\cdot \sum_{i \in \GSet} \zfrac{\size{\bar{\cZ}^+_i}}{2^{\ell}}\\
		&= \frac{0.009}{4m}\cdot \size{\GSet}\cdot \eex{i \la \GSet}{\zfrac{\size{\bar{\cZ}_i^+}}{2^{\ell}}}\\
		&\geq \frac{\eps k}{1800 \cdot m}
	\end{align*}
	\begin{align*}
		\implies \Unf[W] \leq e^{-\frac{\eps k}{1800 \cdot m}} \leq (1-\eps)^{\frac{\eps k}{1800 \cdot m}},
	\end{align*}
	where the first inequality holds from \cref{eq:bad_events:Z_i:1} by \cref{fact:prelim:diver-properties} (data-processing), the third one holds by \cref{fact:prelim:bernoulli-div-est}, the fourth one holds since $\size{\GSet} \geq \zfrac{k}{2}$ and $\eex{i \la \GSet}{\zfrac{\size{\bar{\cZ}_i^+}}{2^{\ell}}} \geq \frac{\eps}{2\lambda}$ and the last one holds since $\eps \in [0,\frac12]$.  Otherwise, the second bound holds and we obtain that
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \sum_{i \in \GSet} \frac{0.9}{m}\cdot \re{\Idl_{Z_i | X_{1,i}=1}(\bar{\cZ}_i^-)}{\Unf_{Z_i}(\bar{\cZ}_i^-)}\\
		&> \sum_{i \in \GSet} \frac{0.9}{m}\cdot \re{(1 - 0.1)\cdot \zfrac{\size{\bar{\cZ}^-_i}}{2^{\ell}}}{\zfrac{\size{\bar{\cZ}^-_i}}{2^{\ell}}}\\
		&\geq \frac{0.9 \cdot 0.1^2}{4m}\cdot \sum_{i \in \GSet} \zfrac{\size{\bar{\cZ}^-_i}}{2^{\ell}}\\
		&= \frac{0.009}{4m}\cdot \size{\GSet}\cdot  \eex{i \la \GSet}{ \zfrac{\size{\bar{\cZ}^-_i}}{2^{\ell}}}\\
		&\geq \frac{\eps k}{1800 \cdot m}
	\end{align*}
	\begin{align*}
		\implies \Unf[W] \leq e^{-\frac{\eps k}{1800 \cdot m}} \leq (1-\eps)^{\frac{\eps k}{3600 \cdot m}}
	\end{align*}
\end{proof}

The proof of \cref{claim:bad_events:main-lemma-D-part} now trivially follows by  \cref{corollary:bad_events:rho-zero,claim:bad_events:Z_i}.


\begin{claim}[Restatement of \cref{claim:bad_events:main-lemma-D-part}]
	\MainLemmaDpart
\end{claim}

\begin{proof}
	Assume that $\size{\cD} \leq (1-\zfrac{\eps}{\lambda}) k\cdot 2^{\ell}$ for some constant $\lambda > 0$ and recall that $\cD = \set{(i,z) \in [k] \times \zo^{\ell} \colon (i,z) \in \GSet \times \cZ_i}$. Compute
	\begin{align*}
		1-\zfrac{\eps}{\lambda}
		&\geq \frac{\size{\cD}}{k\cdot 2^{\ell}}\\
		&= \ppr{(i,z) \la [k]\times \zo^{\ell}}{(i,z) \in \GSet \times \cZ_i}\\
		&= \frac{\size{\GSet}}{k} \cdot \eex{i \la \GSet}{\frac{\size{\cZ_i}}{2^{\ell}}}.
	\end{align*}
	Therefore, it must holds that $\frac{\size{\GSet}}{k} \leq 1 - \frac{\eps}{2\lambda}$ or $\eex{i \la \GSet}{\frac{\size{\cZ_i}}{2^{\ell}}} \leq 1 - \frac{\eps}{2\lambda}$ and we conclude from \cref{corollary:bad_events:rho-zero,claim:bad_events:Z_i} that $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' m}}$ by choosing $\lambda' = \max\set{c,c'}$ where $c$ is the constant $\lambda'(2\lambda)$ of \cref{corollary:bad_events:rho-zero} and $c'$ is the constant $\lambda'(2\lambda)$ of \cref{claim:bad_events:Z_i}.
\end{proof}

\subsubsection{Proving \texorpdfstring{\cref{claim:bad_events:main-lemma-easy-jumps}}{the easy jumps case}}\label{sec:bad_events:main-lemma-easy-jumps}

Before proving \cref{claim:bad_events:main-lemma-easy-jumps}, we first state and prove some useful facts about the $\set{\gamma_{j,i}}$ and $\set{\rho_{j,i}}$ measurements when drawing $Z^k X^{(m+1)\times k}$ from $\Idl$ (done in Sections \ref{sec:bad_events:facts_about_gammas} and \ref{sec:bad_events:facts_about_rhos}, respectively), and the proof of \cref{claim:bad_events:main-lemma-easy-jumps} which follows from these facts is given in Section~\ref{sec:bad_events:easy-jumps:putting-it-together}.

\paragraph{Facts About the $\set{\gamma_{j,i}}$ measurements}\label{sec:bad_events:facts_about_gammas}

The following claim connects the jumps in the measurements $\set{\gamma_{j,i}}_{j\in [m+1],i \in [k]}$ (over $\Idl$) with $\Unf[W]$.

\begin{claim}\label{claim:bad_events:gamma}
	It holds that
	$$\log{\frac1{\Unf[W]}}
	\geq \frac1{4m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \min\set{\size{\gamma_{j,i}}, \gamma_{j,i}^2} \cdot \mathds{1}\set{1 \notin X_{<j,i}}},$$
	where $\gamma_{j,i} = \gamma_{j,i}(Z^k X^{k}_{<j})$.
\end{claim}
\begin{proof}
	Compute
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \re{\Idl_{Z^k X^{(m+1) \times k}}}{\Unf_{Z^k X^{(m+1) \times k}}}\\
		&\geq \sum_{j=1}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\Idl_{X^k_j | Z^k X^k_{<j}}}{\Unf_{X^k_j | Z^k X^k_{<j}}}}\\
		&= \sum_{j=1}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\Idl_{X^k_j | Z^k X^k_{<j}}}{\prod_{i=1}^{k} \Unf_{X_{j,i} | Z^k X^k_{<j}}}}\\
		&\geq \sum_{i=1}^k \sum_{j=1}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\Idl_{X_{j,i} | Z^k X^k_{<j}}}{\Unf_{X_{j,i} | Z^k X^k_{<j}}}}\\
		&= \sum_{i=1}^k \sum_{j=1}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\frac{1 + \gamma_{j,i}}{m}}{\frac1{m}} \cdot \mathds{1}\set{1 \notin X_{<j,i}}}\\
		&\geq \frac1{4m}\cdot \sum_{i=1}^k \sum_{j=1}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j}}}{\min\set{\size{\gamma_{j,i}}, \gamma_{j,i}^2} \cdot \mathds{1}\set{1 \notin X_{<j,i}}}\\
		&= \frac1{4m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \min\set{\size{\gamma_{j,i}}, \gamma_{j,i}^2} \cdot \mathds{1}\set{1 \notin X_{<j,i}}},
	\end{align*}
	where the first inequality holds by \cref{fact:kl-divergence:diver-cond-on-event}, the second one holds by the chain-rule property of KL-Divergence (\cref{fact:prelim:diver-properties}(\ref{fact:diver-properties:item:chain-rule})), the third one holds by the product case of chain-rule (\cref{fact:prelim:diver-properties}(\ref{fact:diver-properties:item:chain-rule})) and the last one holds by \cref{fact:prelim:bernoulli-div-est}.
\end{proof}

As a first corollary of \cref{claim:bad_events:gamma}, we obtain an upper bound on the sum of squares of ``small'' jumps in the values of $\set{\gamma_{j,i}}_{j\in [m+1],i \in [k]}$ (over $\Idl$) in case $\Unf[W]$ is high enough. 

\begin{corollary}\label{corollary:bad_events:gamma:small}
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1}} \geq \zfrac{\eps k}{\lambda}$ for $\gamma_{j,i} = \gamma_{j,i}(Z^k X^k_{<j})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{corollary}
\begin{proof}
	Immediately follows by \cref{claim:bad_events:gamma}.
\end{proof}

As a second corollary of \cref{claim:bad_events:gamma}, we obtain an upper bound on the sum of ``large'' jumps in the values of $\set{\gamma_{j,i}}_{j\in [m+1],i \in [k]}$ (over $\Idl$) in case $\Unf[W]$ is high enough.

\begin{corollary}\label{corollary:bad_events:gamma:large-and-J}
	For any constants $\lambda > 0$ and $c \in (0,1)$ there exists a constant $\lambda' > 0$ such that if one of the following holds:
	\begin{enumerate}
		\item $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \size{\gamma_{j,i}} \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\size{\gamma_{j,i}} > c}} \geq \zfrac{\eps k}{\lambda}$, or\label{item:bad_events:gamma:large}
		\item $\eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\jmp^{\size{\gamma} > c}_i < \infty}} \geq \zfrac{\eps k}{\lambda}$, \label{item:bad_events:gamma:J}
	\end{enumerate}
	for $\gamma_{j,i} = \gamma_{j,i}(Z^k X^k_{<j})$ and $\jmp^{\size{\gamma} > c}_i = \jmp^{\size{\gamma} > c}_i(Z^k X^{(m+1) \times k})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{corollary}
\begin{proof}
	If \cref{item:bad_events:gamma:large} holds, the proof follows by \cref{claim:bad_events:gamma} and by the assumption that $\eps \in [0,\frac12]$, since for any $i \in [k]$, $j \in [m+1]$ and $\tau_j = z^k x^k_{<j} \in \Supp(\Idl_{Z^k X^k_{<j}})$ it holds that 
	\begin{align*}
		\min\set{\size{\gamma_{j,i}(\tau_j)}, \gamma_{j,i}(\tau_j)^2} \cdot \mathds{1}\set{1 \notin X_{<j,i}}
		\geq c\cdot \size{\gamma_{j,i}(\tau_j)} \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\size{\gamma_{j,i}(\tau_j)} > c}
	\end{align*}
	If \cref{item:bad_events:gamma:J} holds, the proof follows by \cref{item:bad_events:gamma:large} since for any $z^k x^{(m+1)\times k} \in \Supp(\Idl)$ it holds that
	\begin{align*}
		\mathds{1}\set{\jmp^{\size{\gamma} > c}_i(z^k x^{(m+1)\times k}) < \infty} 
		&= \sum_{j=1}^{m+1} \mathds{1}\set{\jmp^{\size{\gamma} > c}_i(z^k x^{k}_{<j}) = j}\\
		&\leq \frac1{c} \cdot \sum_{j=1}^{m+1} \size{\gamma_{j,i}(z^k x^{k}_{<j})}\cdot \mathds{1}\set{\jmp^{\size{\gamma} > c}_i(z^k x^{k}_{<j}) = j}\\
		&\leq \frac1{c} \cdot \sum_{j=1}^{m+1} \size{\gamma_{j,i}(z^k x^{k}_{<j})}\cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\size{\gamma_{j,i}(z^k x^{k}_{<j})} > c}
	\end{align*}
\end{proof}

As a trivial corollary of \cref{corollary:bad_events:gamma:large-and-J}, we now prove \cref{claim:bad_events:large-gammas}.

\begin{corollary}[restatement of \cref{claim:bad_events:large-gammas}]\label{corollary:bad_events:large-gammas-rest}
	\LargeGammasClaim
\end{corollary}
\begin{proof}
	Immediately follows by \cref{corollary:bad_events:gamma:large-and-J}(\ref{item:bad_events:gamma:large}) \wrt $c=1$.
\end{proof}


\paragraph{Facts About the $\set{\rho_{j,i}}$ measurements}\label{sec:bad_events:facts_about_rhos}
The following claim connects the jumps in the measurements $\set{\rho_{j,i}}_{j\in [m+1],i \in [k]}$ (over $\Idl$) with $\Unf[W]$.

\begin{claim}\label{claim:bad_events:rho}
	It holds that
	\begin{align*}
		\log{\frac1{\Unf[W]}} \geq \frac1{4m}(1-\frac1m)\cdot \max\set{S_{even},S_{odd}},
	\end{align*}
	where $S_{\nu} \eqdef \eex{\Idl}{\sum_{i=1}^k \sum_{j \in [m+1]\bigcap \N_{\nu}} \min\set{\size{\rho_{j,i}}, \rho_{j,i}^2} \cdot \mathds{1}\set{1 \notin X_{<j,i}}}$ for $\nu \in \set{even,odd}$ and $\rho_{j,i} = \rho_{j,i}(Z^k X^{k}_{<j})$.
\end{claim}
\begin{proof}
	Fix $\nu \in \set{even,odd}$ and compute
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \re{\Idl_{Z^k X^{(m+1) \times k}}}{\Unf_{Z^k X^{(m+1) \times k}}}\\
		&\geq \sum_{j \in [m+1]\cap \N_{\nu}} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\Idl_{X^k_j X^k_{j+1} | Z^k X^k_{<j}}}{\Unf_{X^k_j X^k_{j+1} | Z^k X^k_{<j}}}}\\
		&\geq \sum_{j \in [m+1]\cap \N_{\nu}} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\Idl_{X^k_{j+1} | Z^k X^k_{<j}}}{\Unf_{X^k_{j+1} | Z^k X^k_{<j}}}}\\
		&= \sum_{j \in [m+1]\cap \N_{\nu}} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\Idl_{X^k_{j+1} | Z^k X^k_{<j}}}{\prod_{i=1}^{k } \Unf_{X_{j+1,i} | Z^k X^k_{<j}}}}\\
		&\geq \sum_{i=1}^k \sum_{j \in [m+1]\cap \N_{\nu}} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\Idl_{X_{j+1,i} | Z^k X^k_{<j}}}{\Unf_{X_{j+1,i} | Z^k X^k_{<j}}}}\\
		&=  \sum_{i=1}^k \sum_{j \in [m+1]\cap \N_{\nu}} \eex{\Idl_{Z^k X^{k}_{<j}}}{\re{\frac{1+\rho_{j,i}}m(1-\frac1{m})}{\frac1{m}(1-\frac1{m})} \cdot \mathds{1}\set{1 \notin X_{<j,i}}}\\
		&\geq \sum_{i=1}^k \sum_{j \in [m+1]\bigcap \N_{\nu}}  \eex{\Idl_{Z^k X^k_{<j}}}{ \frac1{4m}(1-\frac1m)\cdot \min\set{\size{\rho_{j,i}}, \rho_{j,i}^2} \cdot \mathds{1}\set{1 \notin X_{<j,i}}}\\
		&= \frac1{4m}(1-\frac1m)\cdot  S_{\nu},
	\end{align*}
	where the first inequality holds by \cref{fact:kl-divergence:diver-cond-on-event}, the second one holds by the chain-rule property of KL-Divergence (\cref{fact:prelim:diver-properties}(\ref{fact:diver-properties:item:chain-rule})), the fourth holds by the product case of chain-rule (\cref{fact:prelim:diver-properties}(\ref{fact:diver-properties:item:chain-rule})) and the last one holds by \cref{fact:prelim:bernoulli-div-est}.
\end{proof}

As a first corollary of \cref{claim:bad_events:rho}, we obtain an upper bound on the sum of squares of ``small'' jumps in the values of $\set{\rho_{j,i}}_{j\in [m+1],i \in [k]}$ (over $\Idl$) in case $\Unf[W]$ is high enough.

\begin{corollary}\label{claim:bad_events:rho:small}
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \rho_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\rho_{j,i} \leq 1}} \geq \zfrac{\eps k}{\lambda}$ for $\rho_{j,i} = \rho_{j,i}(Z^k X^k_{<j})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{corollary}
\begin{proof}
	Assume that $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \rho_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\rho_{j,i} \leq 1}} \geq \zfrac{\eps k}{\lambda}$ for some constant $\lambda > 0$. Since for any $i \in [k]$, $j \in [m+1]$ and $\tau_j = z^k x^k_{<j} \in \Supp(\Idl_{Z^k X^k_{<j}})$ it holds that $$\min\set{\size{\rho_{j,i}(\tau_j)}, \rho_{j,i}^2(\tau_j)} \cdot \mathds{1}\set{1 \notin X_{<j,i}} \geq \rho_{j,i}^2(\tau_j) \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\rho_{j,i}(\tau_j) \leq 1},$$ our assumption yields that there exists $\nu \in \set{even,odd}$ such that $S_{\nu} \eqdef \eex{\Idl}{\sum_{i=1}^k \sum_{j \in [m+1]\bigcap \N_{\nu}} \min\set{\size{\rho_{j,i}}, \rho_{j,i}^2} \cdot \mathds{1}\set{1 \notin X_{<j,i}}} \geq \frac{\eps k}{2\lambda}$. The proof then immediately follows by \cref{claim:bad_events:rho} and by the assumption that $\eps \in [0,\frac12]$.
\end{proof}

As a second corollary of \cref{claim:bad_events:rho}, we obtain an upper bound on the sum of ``large'' jumps in the values of $\set{\rho_{j,i}}_{j\in [m+1],i \in [k]}$ (over $\Idl$) in case $\Unf[W]$ is high enough.

\begin{corollary}\label{corollary:bad_events:rho:large-and-J}
	For any constants $\lambda > 0$ and $c \in (0,1)$ there exists a constant $\lambda' > 0$ such that
	if one of the following holds:
	\begin{enumerate}
		\item $\sum_{i=1}^k \sum_{j=1}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j}}}{\size{\rho_{j,i}} \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\size{\rho_{j,i}} > c}} \geq \zfrac{\eps k}{\lambda}$, or\label{item:bad_events:rho:large}
		\item $\eex{\Idl_{Z^k X^{(m+1) \times k}}}{\sum_{i=1}^k  \mathds{1}\set{\jmp^{\size{\rho} > c}_i < \infty}} \geq \zfrac{\eps k}{\lambda}$,\label{item:bad_events:rho:J}
	\end{enumerate}
	for $\rho_{j,i} = \rho_{j,i}(Z^k X^k_{<j})$ and $ \jmp^{\size{\rho} > c}_i = \jmp^{\size{\rho} > c}_i(Z^k X^{m \times k})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{corollary}
\begin{proof}
	If \cref{item:bad_events:rho:large} holds, then there exists $\nu \in \set{even,odd}$ with
	\begin{align*}
		\sum_{i=1}^k \sum_{j \in [m+1]\bigcap \N_{\nu}} \eex{\Idl_{Z^k X^{k}_{<j}}}{\size{\rho_{j,i}} \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\size{\rho_{j,i}} > c}} \geq \frac{\eps k}{2\lambda},
	\end{align*}
	and the proof follows by \cref{claim:bad_events:rho} and by the assumption that $\eps \in [0,\frac12]$, since for any $i \in [k]$, $j \in [m+1]$ and $\tau_j \in \Supp(\Idl_{Z^k X^{k}_{<j}})$ it holds that
	\begin{align*}
		\min\set{\size{\rho_{j,i}(\tau_j)}, \rho_{j,i}^2(\tau_j)} \cdot \mathds{1}\set{1 \notin X_{<j,i}} \geq c \cdot \size{\rho_{j,i}(\tau_j)} \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\size{\rho_{j,i}(\tau_j)} > c}.
	\end{align*}
	If \cref{item:bad_events:rho:J} holds, then the proof follows by \cref{item:bad_events:rho:large} since for any $z^k x^{(m+1)\times k} \in \Supp(\Idl)$ it holds that
	\begin{align*}
		\mathds{1}\set{\jmp^{\size{\rho} > c}_i(z^k x^{(m+1)\times k}) < \infty} 
		&= \sum_{j=1}^{m+1} \mathds{1}\set{\jmp^{\size{\rho} > c}_i(z^k x^{k}_{<j}) = j}\\
		&\leq \frac1{c} \cdot \sum_{j=1}^{m+1} \size{\rho_{j,i}(z^k x^{k}_{<j})}\cdot \mathds{1}\set{\jmp^{\size{\rho} > c}_i(z^k x^{k}_{<j}) = j}\\
		&\leq \frac1{c} \cdot \sum_{j=1}^{m+1} \size{\rho_{j,i}(z^k x^{k}_{<j})}\cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\size{\rho_{j,i}(z^k x^{k}_{<j})} > c}
	\end{align*}
\end{proof}


\paragraph{Putting it Together}\label{sec:bad_events:easy-jumps:putting-it-together}

We are finally ready to prove \cref{claim:bad_events:main-lemma-easy-jumps}

\begin{claim}[Restatement of \cref{claim:bad_events:main-lemma-easy-jumps}]
	\MainLemmaEasyJumps
\end{claim}
\begin{proof}
	Recall that $\jumps^{\nu}(\tau) = \sum_{i=1}^k \mathds{1}\set{\jmp^{\size{\nu} > 0.1}_i(\tau) < \infty}$, for any $\nu \in \set{\gamma,\rho}$ and $\tau \in \Supp(\Idl)$. Therefore the proof immediately follows by \cref{corollary:bad_events:gamma:large-and-J}(\ref{item:bad_events:gamma:J}) and \cref{corollary:bad_events:rho:large-and-J}(\ref{item:bad_events:rho:J}).
\end{proof}




\subsubsection{Proving \texorpdfstring{\cref{claim:bad_events:main-lemma-hard-jumps}}{the hard jumps case}}\label{sec:bad_events:main-lemma-hard-jumps}

In this section we prove \cref{claim:bad_events:main-lemma-hard-jumps}, restated for convenience below.

\begin{claim}[Restatement of \cref{claim:bad_events:main-lemma-hard-jumps}]
	\MainLemmaHardJumps
\end{claim}

Proving \cref{claim:bad_events:main-lemma-hard-jumps} is the most challenging part in the proof of \cref{lemma:bad_events:main-lemma}. Unlike the $\set{\gamma_{j,i}}$ and $\set{\rho_{j,i}}$ measurements which are directly connected to $\Unf[W]$ (as we proved in \cref{claim:bad_events:gamma,claim:bad_events:rho}), the connection between the $\set{\aval_{j,i}}$ measurements and $\Unf[W]$ is less clear. Recall that the values $\set{\aval_{j,i}}$ comes from the change in the distribution of $I$ in $Q$ given a history $Z^k X^k_{<j}$, as stated in \cref{claim:PR_Thm:I_dist}:
\begin{align*}
	\Rll_{I | Z^k X_{<j}^k, I \in \mathcal{G}_\tau}(i | z^k x_{<j}^k) = \frac{\aval_{j,i}(z^k x_{<j}^k)}{\sum_{i' \in \mathcal{G}_\tau} \aval_{j,i'}(z^k x_{<j}^k)}.
\end{align*}
Proving \cref{claim:bad_events:main-lemma-hard-jumps} requires a very deep understanding of these measurements, and therefore, we start by presenting the high level plan of this complicated part.

\paragraph{High-Level Plan}\label{sec:bad_events:a_values:high_level_plan}

The goal of this section is to understand the distribution of $\Rll_{I|Z^k X^k_{<j}}$ for every $j \in [m+1]$ when $Z^k X^k_{<j}$ is drawn from $\Idl_{Z^k X^k_{<j}}$. The main idea for proving \cref{claim:bad_events:main-lemma-hard-jumps} is to show that in expectation (over $\Idl$), the distributions $\set{\Rll_{I|Z^k X^k_{<j}}}_{j=1}^{m+1}$ might behave badly over a small set of columns (\ie columns $i \in[k]$ which has large ``jumps'' in their $\aval_{j,i}$ value for some $j \in [m+1]$), but conditioned on the event that $I$ is not in the ``bad'' set, it remains close to uniform over the ``good'' columns. Informally, \cref{claim:bad_events:main-lemma-hard-jumps} states that in expectation over $\Idl$, $(1-o(\eps))k$ of the columns $i \in [k]$ are ``good'' which means that they have $\aval_{j,i} \in [0.01,10]$ for all $j \in [m+1]$. Intuitively, this means that by taking uniformly $I \la [k]$ at the beginning (as done in $\Rll$), we hit a potential "bad" column only with probability $o(\eps)$, and conditioned on hitting the ''good'' set, the distribution of $Q_{I | Z^k X^k_{<j}}$ remains ''close enough'' to uniform over the ''good'' set of columns (\cref{claim:PR_Thm:I_dist}). Now, recall that

\begin{align}\label{eq:bad_events:a_values:def}
	\aval_{j,i} =\frac{\Unf_{Z_{i}}(z_i)}{\Idl_{Z_{i}}(z_i)} \cdot \frac{\Idl_{X_{1,i} | Z^k}(1 | z^k)}{\Idl_{X_{1,i} | Z_{i}}(1 | z_{i})} \cdot \prod_{j'=2}^{j} \left(1+\beta_{j',i}(z^k x_{<j'}^k)\right).
\end{align}

In Section~\ref{sec:bad_events:a_values:first_terms} we handle the first two terms of (\ref{eq:bad_events:a_values:def}) which captures the effect of choosing $z^k \sim \Idl_{Z^k}$ on the distribution $\Rll_{I|Z^k=z^k}$. This is done by showing (using standard arguments) that if $\Unf[W]$ is high enough, then in expectation (over $z^k \sim \Idl_{Z^k}$), most columns $i \in [k]$ (all but $o(\eps k)$) have $\frac{\Unf_{Z_{i}}(z_i)}{\Idl_{Z_{i}}(z_i)} \approx 1$ and $\frac{\Idl_{X_{1,i} | Z^k}(1 | z^k)}{\Idl_{X_{1,i} | Z_{i}}(1 | z_{i})} \approx 1$.  In Section~\ref{sec:bad_events:a_values:the_martingale_seq} we handle the complex part of the proof by showing that if $\Unf[W]$ is high enough, then in expectation (over $z^k x^{(m+1)\times k} \sim \Idl$), most active columns $i \in [k]$ (all but $o(\eps k)$) have values $\set{\prod_{j'=2}^{j}(1 + \bbeta_{j',i})}_{j \in [m+1]}$ bounded between two constants (inside the interval $[0.01,10]$), where the above product captures the effect of choosing $x^{k}_{<j} \sim \Idl_{X^k_{<j} | Z^k = z^k}$ on $\Rll_{I|(Z^k X^k_{<j})=z^k x^k_{<j}}$ for any fixing of $z^k$. We now focus on giving the high level parts of the ideas in Section~\ref{sec:bad_events:a_values:the_martingale_seq}.  Given $\tau_j = \tau_{j-1} x^k_{j-1} = z^k x^k_{<j}$, recall that
\begin{align*}
	\bbeta_{j,i}(\tau_j) = \frac{\Idl_{X_{j,i} | Z^k X_{<j}^k}(1 | \tau_j)}{\Idl_{X_{j,i} | Z^k X_{<j-1}^k}(1 | \tau_{j-1})} - 1
\end{align*}
and observe that
\begin{align*}
	\eex{\Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\bbeta_{j,i}(\tau_{j-1} X^k_{j-1})}
	= \frac{\eex{\Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\Idl_{X_{j,i} | Z^k X_{<j}^k}(1 | \tau_{j-1} X^k_{j-1})}}{\Idl_{X_{j,i} | Z^k X_{<j-1}^k}(1 | \tau_{j-1})} - 1 = 0.
\end{align*}

Namely, for every $i \in [k]$, the sequence $\set{\bbeta_{j,i}}_{j=2}^{m+1}$ is a martingale difference sequence with respect to $\set{\Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}}_{j=2}^{m+1}$ for any fixing of $Z^k$. Therefore, if we could prove that for most active columns $i \in [k]$ (all but $o(\eps k)$) it holds that $\eex{\Idl}{\sum_{j=2}^{m+1} \bbeta_{j,i}^2} \leq o(\eps)$, then we could apply \cref{fact:prelim:martingales:week_concent} for obtaining that in expectation over $\Idl$,  there are at least $(1 - o(\eps))k$ columns $i \in [k]$ in which all their partial sums $\set{\sum_{j'=2}^{j} \bbeta_{j',i}}_{j=2}^{m+1}$ are bounded in an interval of the form $[-O(1),O(1)]$. For such columns, we could bound the values $\set{\prod_{j'=2}^{j}(1 + \bbeta_{j',i})}_{j \in [m+1]}$ since $\prod_{j'=2}^{j}(1 + \bbeta_{j',i}) \approx \exp\paren{\sum_{j'=2}^j \bbeta_{j',i}}$ (assuming that all values $\set{\bbeta_{j,i}}_{j=2}^{m+1}$ are small). The problem is that the above claim is incorrect. Namely, even if $\Unf[W] = 1$ (\ie $\Idl = \Unf_{Z^k X^{(m+1) \times k}}$), still we expect to have at least $\Omega(k)$ columns with $\eex{\Idl}{\sum_{j=2}^{m+1} \bbeta_{j,i}^2} \geq \Omega(1)$. In order to see it, fix $j \in [m+1]$ and $\tau_j = z^k x^k_{<j}$ with $1 \notin x^k_{<j-1}$ (\ie active) and observe that in this degenerate case where $\Unf[W] = 1$ (denote as the ``Uniform'' case and denote its $\bbeta_{j,i}$ by $\bbeta_{j,i}^U$), we have
\begin{align*}
	\bbeta_{j,i}^U(\tau_j)
	&= \frac{\Unf_{X_{j,i} | Z^k X_{<j}^k}(1 | \tau_j)}{\Unf_{X_{j,i} | Z^k X_{<j-1}^k}(1 | \tau_{j-1})} - 1\\
	&= \frac{\begin{cases} \frac1{m} & x_{j-1,i}=0 \\ 0 & x_{j-1,i}=1 \end{cases}}{\frac1{m}(1-\frac1{m})} - 1\\
	&= \begin{cases} \frac1{m-1} & x_{j-1,i}=0 \\ -1 & x_{j-1,i}=1,\end{cases}
\end{align*}
Namely, as long there is no value $1$ in the past (\ie $1 \notin x_{<j-1,i}$ for the \jth element), the next element is $-1$ w.p. $\frac1{m}$ and $\frac1{m-1}$ otherwise. Since we expected that at least $\Omega(k)$ of the columns $i \in [k]$ have $x_{\leq m+1,i} = 0^{m+1}$, these sequences have $\sum_{j=2}^{m+1} (\bbeta_{j,i}^U)^2  \geq \Omega(1)$, and therefore, not bounded by $o(\eps)$. Yet, this sequences still behave nicely in a sense that the values $\set{\prod_{j'=2}^{j}(1 + \bbeta_{j',i}^U)}_{j=2}^{m+1} = \set{(1 + \frac1{m-1})^{j-1}}_{j=2}^{m+1}$ are always bounded in the interval $[1,4]$ in case $x_{\leq m+1, i} = 0^{m+1}$. Back to the general case where $\Unf[W] \leq 1$, the above observation leads us to explore the sequences $\set{\hbeta_{j,i}}$ for $\hbeta_{j,i} = \bbeta_{j,i} - \bbeta_{j,i}^U$ and prove that if $\Unf[W]$ is high enough, then for most active  columns $i \in [k]$ we have $\eex{\Idl}{\sum_{j=2}^{m+1} \hbeta_{j,i}^2} \leq o(\eps)$. The first problem is that now this is not necessarily a martingale difference sequence anymore. Therefore, we transform it into a martingale by defining $\hbeta_{j,i} = \bbeta_{j,i} - \bbeta_{j,i}^U + \mu_{j-1,i}^U$ where $ \mu_{j-1,i}^U(\tau_{j-1}) = \eex{\Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\bbeta_{j,i}^U(\tau_{j-1} X^k_{j-1})}$. The second problem is that in the general case, there might be large  jumps in the value of $\bbeta_{j,i}$ (\ie $\bbeta_{j,i}$ might be larger than 1 and even $\approx m$). In order to see why this is a problem, consider the case where it always holds that the values $\set{\rho_{j,i}}$ are zeros, and therefore, if $\bbeta_{j,i} = \frac{m}{m-1} \cdot \frac{1 + \gamma_{j,i}}{1 + \rho_{j-1,i}} - 1 = \frac{m}{m-1} (\gamma_{j,i} - \frac1{m}) >> 1$ then $\bbeta_{j,i} \approx \gamma_{j,i}$.  Hence, if we could prove that high enough $\Unf[W]$ implies $\ex{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i}^2 \cdot \mathds{1}\set{\gamma_{j,i} > 1}} < o(\eps k)$, then we could handle the $\bbeta_{j,i}^2$'s in case of large jumps. However, the above bound is incorrect and by \cref{claim:bad_events:large-gammas} we only know that high enough $\Unf[W]$ implies $\ex{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i} \cdot \mathds{1}\set{\gamma_{j,i} > 1}} < o(\eps k)$ (\ie we loose the squares in the large jumps case). We solve this issue by cutting the large jumps and defining $\hbeta_{j,i} = \bbeta_{j,i}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1} + \xi_{j-1,i} -  \bbeta^U_{j,i} + \mu^U_{j-1,i}$ where $\xi_{j-1,i}(\tau_{j-1}) = \eex{x^k_{j-1} \sim \Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\bbeta_{j,i}(\tau_{j-1} x^k_{j-1}) \cdot \mathds{1}\set{\gamma_{j,i}(\tau_{j-1} x^k_{j-1}) > 1}}$ is added in order to preserve the martingale property of these sequences. Finally, by \cref{claim:bad_events:main-lemma-easy-jumps,corollary:bad_events:xi:second}, we actually expect that if $\Unf[W]$ is high enough, then for most active columns $i \in [k]$ (all but $o(\eps k)$) there are no jumps in the values of $\set{\gamma_{j,i}}$, $\set{\rho_{j,i}}$ and $\set{\xi_{j,i}}$ and in our analysis we use it by zeroing the sequence $\set{\hbeta_{j,i}}_{j=2}^{m+1}$ in some round $j$ if there was some large jump in one of measurements of the first $j-1$ rounds (denote this ``bad'' event by $\Good_{j-1,i} = 0$). Moreover, since we do not expect such jumps for most active columns, then it can be shown that for such good column $i \in [k]$, the sequence $\set{\hbeta_{j,i}}_{j=2}^{m+1}$ which we finally can bound using a fact about martingales, is close enough to the desired sequence $\set{\bbeta_{j,i}}_{j=2}^{m+1}$ and the proof follows.

\paragraph{Round  Zero}\label{sec:bad_events:a_values:first_terms}

The following claim states that if $\Unf[W]$ is high enough, then in expectation (over $z^k \sim \Idl_{Z^k}$), most columns $i \in [k]$ (all but $o(\eps k)$) have $\frac{\Unf_{Z_{i}}(z_i)}{\Idl_{Z_{i}}(z_i)} \approx 1$.


\begin{claim}\label{claim:bad_events:a_first_term}
	For every two constants $\lambda > 0$ and $c \in (0,1)$ there exists a constant $\lambda' > 0$ such that if $\eex{z^k \sim \Idl_{Z^k}}{\sum_{i=1}^k \mathds{1}\set{\Idl_{Z_i}(z_i) \notin (1 \pm c) \cdot \Unf_{Z_i}(z_i)}}> \zfrac{\eps k}{\lambda}$, then $\Unf[W] \leq (1-\eps)^{\zfrac{k}{\lambda'}}$.
\end{claim}

\begin{proof}
	We first handle the case $\eex{z^k \sim \Idl_{Z^k}}{\sum_{i=1}^k \mathds{1}\set{\Idl_{Z_i}(z_i) > (1 + c) \cdot \Unf_{Z_i}(z_i)}}> \frac{\eps k}{2 \lambda}$. Let $p_i \eqdef \ppr{z \sim \Idl_{Z_i}}{\Idl_{Z_i}(z) > (1+c) \cdot \Unf_{Z_i}(z)}$ and $q_i \eqdef \ppr{z \sim \Unf_{Z_i}}{\Idl_{Z_i}(z) > (1+c) \cdot \Unf_{Z_i}(z)}$. Recall that by assumption, $\sum_{i=1}^k p_i \geq \frac{\eps k}{2 \lambda}$ and observe that for any $i \in [k]$ it holds that $q_i \leq \frac{p_i}{1+c}$. The proof then follows since
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \re{\Idl_{Z^k}}{\Unf_{Z^k}}
		= \re{\Idl_{Z^k}}{\prod_{i=1}^{k} \Unf_{Z_i}}\\
		&\geq \sum_{i=1}^k \re{\Idl_{Z_i}}{\Unf_{Z_i}}
		\geq \sum_{i=1}^k \re{p_i}{q_i}\\
		&\geq \sum_{i=1}^k \re{(1 + c)\frac{p_i}{1+c}}{\frac{p_i}{1+c}}\\
		&\geq \frac{c^2}{4} \cdot \sum_{i=1}^k p_i
		\geq c^2 \cdot \frac{\eps k}{8 \lambda}
	\end{align*}
	\begin{align*}
		\implies \Unf[W] \leq e^{-c^2 \cdot \frac{\eps k}{8 \lambda}} \leq (1-\eps)^{\zfrac{\eps k}{\left(\zfrac{16 \lambda}{c^2}}\right)},
	\end{align*}
	where the first inequality holds by \cref{fact:kl-divergence:diver-cond-on-event}, the second and third one holds by \cref{fact:prelim:diver-properties} (the product case of chain-rule and data-processing, respectively), and the one before last holds by \cref{fact:prelim:bernoulli-div-est}.

	Otherwise, it holds that $\eex{z^k \sim \Idl_{Z^k}}{\sum_{i=1}^k \mathds{1}\set{\Idl_{Z_i}(z_i) < (1 - c) \cdot \Unf_{Z_i}(z_i)}}> \frac{\eps k}{2\lambda}$. In this case we define $p_i \eqdef \ppr{z \sim \Idl_{Z_i}}{\Idl_{Z_i}(z) < (1-c) \cdot \Unf_{Z_i}(z)}$ and $q_i \eqdef \ppr{z \sim \Unf_{Z_i}}{\Idl_{Z_i}(z) < (1 - c) \cdot \Unf_{Z_i}(z)}$ and note that $p_i \leq (1-c) q_i$ and $\sum_{i=1}^k q_i \geq \sum_{i=1}^k p_i \geq \frac{\eps k}{2\lambda}$. The proof then follows since
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \sum_{i=1}^k \re{\Idl_{Z_i}}{\Unf_{Z_i}}
		\geq \sum_{i=1}^k \re{p_i}{q_i}\\
		&\geq \sum_{i=1}^k \re{(1 - c) q_i}{q_i}
		\geq \frac{c^2}{2}\cdot \sum_{i=1}^k q_i\\
		&\geq c^2\cdot \frac{\eps k}{4\lambda}
	\end{align*}
	\begin{align*}
		\implies \Unf[W] \leq e^{-c^2\cdot \frac{\eps k}{4\lambda}} \leq (1-\eps)^{\zfrac{k}{\left(\zfrac{8 \lambda}{c^2}}\right)}
	\end{align*}
\end{proof}

The following claim states that if $\Unf[W]$ is high enough, then in expectation (over $z^k \sim \Idl_{Z^k}$), most columns $i \in [k]$ (all but $o(\eps k)$) have $\frac{\Idl_{X_{1,i} | Z^k}(1 | z^k)}{\Idl_{X_{1,i} | Z_{i}}(1 | z_{i})} \approx 1$

\begin{claim}\label{claim:bad_events:a_sec_term}
	For every two constants $\lambda > 0$ and $c \in (0,1)$ there exists a constant $\lambda' > 0$ such that if $\eex{\Idl_{Z^k}}{\sum_{i=1}^k \mathds{1}\set{\Idl_{X_{1,i} | Z_i}(1) \notin \frac{1 \pm c}m}} \geq \zfrac{\eps k}{\lambda}$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{claim}
\begin{proof}
	Compute
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq  \re{\Idl_{Z^k X^k_1}}{\Unf_{Z^k X^k_1}}
		= \re{\Idl_{Z^k X^k_1}}{\prod_{i=1}^{k} \Unf_{Z_i X_{1,i}}}\\
		&\geq \sum_{i=1}^k \re{\Idl_{Z_i X_{1,i}}}{\Unf_{Z_i X_{1,i}}}
		\geq  \sum_{i=1}^k \eex{\Idl_{Z_i}}{\re{\Idl_{X_{1,i} | Z_i}}{\Unf_{X_{1,i} | Z_i}}}\\
		&\geq \sum_{i=1}^k \eex{\Idl_{Z_i}}{\re{\Idl_{X_{1,i} | Z_i}}{\Unf_{X_{1,i} | Z_i}} \cdot \mathds{1}\set{\Idl_{X_{1,i} | Z_i}(1) \notin \frac{1 \pm c}m}}\\
		&\geq \frac{c^2}{4m} \cdot \eex{\Idl_{Z_i}}{\sum_{i=1}^k \mathds{1}\set{\Idl_{X_{1,i} | Z_i}(1) \notin \frac{1 \pm c}m}}\\
		&\geq c^2\cdot \frac{\eps k}{4\lambda \cdot m}
	\end{align*}
	\begin{align*}
		\implies \Unf[W] \leq e^{-c^2\cdot \frac{\eps k}{4\lambda \cdot m}} \leq (1-\eps)^{\frac{k}{\left(\zfrac{8\lambda}{c^2}\right) \cdot m}},
	\end{align*}
	where the first inequality holds by \cref{fact:kl-divergence:diver-cond-on-event}, the second and third ones hold by \cref{fact:prelim:diver-properties} (chain-rule) and the one before last holds by \cref{fact:prelim:bernoulli-div-est} since $\Unf_{X_{1,i} | Z_i}(1) = \frac1{m}$.
\end{proof}

\paragraph{Rounds $1$ to $m+1$}\label{sec:bad_events:a_values:the_martingale_seq}

As mentioned in Section~\ref{sec:bad_events:a_values:high_level_plan}, the goal of this section is to prove that if $\Unf[W]$ is high enough, then for most active columns $i \in [k]$ (all but $o(\eps k)$) it holds that the values $\set{\prod_{j'=2}^{j}(1 + \bbeta_{j',i})}_{j=2}^{m+1}$ are bounded between two constants, and then using Section~\ref{sec:bad_events:a_values:first_terms} we deduce \cref{claim:bad_events:main-lemma-hard-jumps}. In \cref{fig:bad_events:add_measur} we present the formal definitions of the new variables that are mentioned in Section~\ref{sec:bad_events:a_values:high_level_plan}.

\begin{table}[ht]
	\begin{center}
		\caption{\label{fig:bad_events:add_measur} Additional Measurements.}
		\begin{tabular}{|c|c|c|}
			\hline
			\textit{Definition} & \textit{Value}\\
			\hline
			$\xi_{j,i}(\tau_j)$ & $\eex{x^k_{j-1} \sim \Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\bbeta_{j,i}(\tau_{j-1} x^k_{j-1}) \cdot \mathds{1}\set{\gamma_{j,i}(\tau_{j-1} x^k_{j-1}) > 1}}$ \\
			\hline
			$\bbeta_{j,i}^U(\tau_j)$ & $\begin{cases} \frac1{m-1} & x_{j-1,i}=0 \\ -1 & x_{j-1,i}=1 \end{cases}$ \\
			\hline
			$\mu_{j,i}^U(\tau_j)$ & $\eex{x^k_{j-1} \sim \Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\bbeta^U_{j,i}(\tau_{j-1} x^k_{j-1})}$ \\
			\hline
			$\Good_{j,i}(\tau_j)$ & $\mathds{1}\set{i \in \GSet^{\gamma}_{\tau_{j}} \cap \GSet^{\rho}_{\tau_{j}}}\cdot \mathds{1}\set{\xi_{j,i} \leq 0.1}$\\
			\hline
			$\hbeta_{j,i}(\tau_j)$ & $\begin{cases} 0 & \Good_{j-1,i}=0 \\ \bbeta_{j,i}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1} + \xi_{j-1,i} -  \bbeta^U_{j,i} + \mu^U_{j-1,i} & \text{Otherwise} \end{cases}$\\
			\hline
		\end{tabular}
	\end{center}
\end{table}

The following claim states basic facts about the new variables.

\begin{claim}[Measurements' Properties]\label{claim:bad_events:list_of_properties}
	For any $\tau_j = \tau_{j-1} x^k_{j-1} = z^k x^{k}_{<j} \in \Supp(\Idl_{Z^k X^k_{<j}})$ it holds that
	\begin{enumerate}
		\item $1 \notin x_{<j-1,i} \implies \mu_{j-1,i}(\tau_{j-1}) = -\frac{\gamma_{j-1,i}(\tau_{j-1})}{m-1}$.\label{item:bad_events:list_of_properties:1}
		\item $\eex{\Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\hbeta_{j,i}(\tau_{j-1} X^k_{j-1})} = 0$.\label{item:bad_events:list_of_properties:2}
		\item $\size{\hbeta_{j,i}(\tau_j)} \leq 7$.\label{item:bad_events:list_of_properties:3}
		\item $\gamma_{j,i}(\tau_j) > 1, \size{\rho_{j-1,i}(\tau_{j-1})} \leq 0.1 \implies \bbeta_{j,i}(\tau_j) \in (0.8\gamma_{j,i}, 4 \gamma_{j,i})$.\label{item:bad_events:list_of_properties:4}
		\item $1 \notin x_{<j,i}, \gamma_{j,i} \leq 1 \implies $ $\gamma_{j,i}(\tau_j) = \frac{m-1}{m} (1 + \rho_{j-1,i}) \left(\hbeta_{j,i} + \frac{\gamma_{j-1,i}}{m-1} - \xi_{j-1,i}\right) + \rho_{j-1,i}$.\label{item:bad_events:list_of_properties:5}
		\item $1 \notin x_{<j,i}, \gamma_{j,i} \leq 1, \size{\rho_{j-1,i}}, \xi_{j,i} \leq 0.1 \implies \gamma_{j,i}^2 \leq \frac1{10} \hbeta_{j,i}^2 - \gamma_{j-1,i}^2 - \xi_{j-1,i} - 3 \rho_{j-1,i}^2$\label{item:bad_events:list_of_properties:6}
	\end{enumerate}
\end{claim}
\begin{proof}
	For property~\ref{item:bad_events:list_of_properties:1}, compute
	\begin{align}
		\mu^U_{j-1,i}(\tau_{j-1})
		&= -1 \cdot \Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(1 | \tau_{j-1}) + \frac1{m-1}\cdot \Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(0 | \tau_{j-1})\\
		&= - \frac{1 + \gamma_{j-1,i}(\tau_{j-1})}{m} + \frac1{m-1}\cdot \left(1 - \frac{1 + \gamma_{j-1,i}(\tau_{j-1})}{m}\right)\nonumber\\
		&= - \frac{\gamma_{j-1,i}(\tau_{j-1})}{m-1}.\nonumber
	\end{align}
	For property~\ref{item:bad_events:list_of_properties:2}, observe that if $\Good_{j-1,i} = 0$ then $\hbeta_{j,i} = 0$ by definition, and otherwise it holds that
	\begin{align*}
		\lefteqn{\eex{x^k_{j-1} \sim \Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau)}{\hbeta_{j,i}(\tau_{j-1} x^k_{j-1})}}\\
		&= \eex{x^k_{j-1}}{\bbeta_{j,i}\cdot \mathds{1}\set{\gamma_{j,i}  \leq 1} + \xi_{j-1,i} -  \bbeta^U_{j,i} + \mu^U_{j-1,i}}\nonumber\\
		&=  \eex{x^k_{j-1}}{\bbeta_{j,i}} \cdot \ppr{x^k_{j-1}}{\gamma_{j,i}  \leq 1} + \eex{x^k_{j-1}}{\bbeta_{j,i}} \cdot \ppr{x^k_{j-1}}{\gamma_{j,i}  > 1} - \eex{x^k_{j-1}}{\bbeta^U_{j,i}} + \eex{x^k_{j-1}}{\bbeta^U_{j,i}}\nonumber\\
		&= \eex{x^k_{j-1} \sim \Idl_{X^k_{j-1} | Z^k X^k_{<j}}(\cdot | \tau_{j-1})}{\bbeta_{j,i}(\tau_{j-1}  x^k_{j-1})}\nonumber\\
		&= \frac{\eex{x^k_{j-1} \sim \Idl_{X^k_{j-1} | Z^k X^k_{<j-1}}(\cdot | \tau_{j-1})}{\Idl_{X_{j,i} | Z^k X^k_{<j}}(1 | \tau_{j-1} x^k_{j-1})}}{\Idl_{X_{j,i} | Z^k X^k_{<j-1}}(1 | \tau_{j-1})} - 1\nonumber\\
		&= 0\nonumber
	\end{align*}
	For property~\ref{item:bad_events:list_of_properties:3}, recall that if $\Good_{j-1,i}(\tau_{j-1}) = 0$ then $\hbeta_{j,i}(\tau_{j}) = 0$ and otherwise
	\begin{align*}
		\size{\hbeta_{j,i}(\tau_j)}
		&\leq \size{\bbeta_{j,i}}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1} + \size{\xi_{j-1,i}} + \size{\bbeta^U_{j,i}} + \size{\mu^U_{j-1,i}}\\
		&\leq \frac{m}{m-1} \cdot \frac{1 + \gamma_{j,i}}{1 + \rho_{j-1,i}}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1} + \xi_{j-1,i} + 2\\
		&\leq 2\cdot \frac{2}{1-0.1} + 0.1 + 2\\
		&\leq 7
	\end{align*}
	For property~\ref{item:bad_events:list_of_properties:4}, recall that $\gamma_{j,i} > 1$ and $\rho_{j-1,i} \leq 0.1$. The upper bound holds since
	\begin{align*}
		\bbeta_{j,i}
		&= \frac{m}{m-1}\cdot \frac{1 + \gamma_{j,i}}{1 + \rho_{j-1,i}} - 1\\
		&\leq 2 \cdot \frac{1 + \gamma_{j,i}}{1 - 0.1} - 1
		< 2.5 \gamma_{j,i} + 1.5
		< 4 \gamma_{j,i}
	\end{align*}
	and the lower bound holds since
	\begin{align*}
		\bbeta_{j,i}
		&= \frac{m}{m-1}\cdot \frac{1 + \gamma_{j,i}}{1 + \rho_{j-1,i}} - 1\\
		&\geq \frac{1 + \gamma_{j,i}}{1 + 0.1} - 1
		> 0.9 \gamma_{j,i} - 0.1
		> 0.8 \gamma_{j,i}
	\end{align*}

	For property~\ref{item:bad_events:list_of_properties:5}, compute
	\begin{align*}
		\gamma_{j,i}(\tau_j)
		&= \frac{m-1}{m} (1+\rho_{j-1,i})(1 + \bbeta_{j,i}) - 1\\
		&= \frac{m-1}{m} (1+\rho_{j-1,i})(1 + \hbeta_{j,i} - \xi_{j-1,i} + \frac1{m-1} + \frac{\gamma_{j-1,i}}{m-1}) - 1\\
		&= \frac{m-1}{m} (\hbeta_{j,i} - \xi_{j-1,i} + \frac{\gamma_{j-1,i}}m) + \frac{m-1}{m} \rho_{j-1,i} (1 + \hbeta_{j,i} - \xi_{j-1,i} + \frac1{m-1} + \frac{\gamma_{j-1,i}}{m-1})\\
		&= \frac{m-1}{m} (1 + \rho_{j-1,i}) \left(\hbeta_{j,i} + \frac{\gamma_{j-1,i}}{m-1} - \xi_{j-1,i}\right) + \rho_{j-1,i}\\
	\end{align*}
	For property~\ref{item:bad_events:list_of_properties:6}, compute
	\begin{align*}
		\gamma_{j,i}(\tau_j)^2
		&=\left(\frac{m-1}{m} (1 + \rho_{j-1,i}) \hbeta_{j,i} +  \bigl((1 + \rho_{j-1,i})\cdot \frac{\gamma_{j-1,i}}{m} - \frac{m-1}{m}(1 + \rho_{j-1,i}) \xi_{j-1,i} + \rho_{j-1,i}\bigr)\right)^2\\
		&\geq \frac12\left(\frac{m-1}{m} (1 + \rho_{j-1,i}) \hbeta_{j,i}\right)^2 - \left((1 + \rho_{j-1,i})\cdot \frac{\gamma_{j-1,i}}{m} - \frac{m-1}{m}(1 + \rho_{j-1,i}) \xi_{j-1,i} + \rho_{j-1,i}\right)^2\\
		&\geq \frac1{10} \hbeta_{j,i}^2 - 3\cdot \left(\frac{(1 + 0.1)^2}{m^2} \gamma_{j-1,i}^2 + (1+0.1)^2 \xi_{j-1,i}^2 + \rho_{j-1,i}^2 \right)\\
		&\geq \frac1{10} \hbeta_{j,i}^2 - \gamma_{j-1,i}^2 - \xi_{j-1,i} - 3 \rho_{j-1,i}^2,
	\end{align*}
	where the first inequality holds by the fact that $(a+b)^2 \geq \frac12 a^2 - b^2$, the second inequality holds by the fact that $(a+b+c)^2 \leq 3(a^2 + b^2 + c^2)$ and by the bound $m \geq 2$ and $\size{\rho_{j-1,i}} \leq 0.1$, and the last one holds since $m \geq 2$ and $0 \leq \xi_{j,i} \leq 0.1$.
\end{proof}

The following claim connects between the measurements $\set{\xi_{j,i}}_{j,i}$ to $\Unf[W]$.

\begin{claim}\label{claim:bad_events:xi}
	It holds that
	\begin{align*}
		\log{\frac1{\Unf[W]}} \geq \frac1{16m} \sum_{i=1}^k \sum_{j=1}^{m} \eex{\Idl_{Z^k X^{k}_{<j}}}{\xi_{j,i} \cdot \mathds{1}\set{\size{\rho_{j,i}} \leq 0.1}},
	\end{align*}
	for $\xi_{j,i} = \xi_{j,i}(Z^k X^{k}_{<j})$ and $\rho_{j,i} = \rho_{j,i}(Z^k X^{k}_{<j})$.
\end{claim}
\begin{proof}
	Compute
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \frac1{4m}\cdot \sum_{i=1}^k \sum_{j=2}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j}}}{\gamma_{j,i} \cdot \mathds{1}\set{\gamma_{j,i}> 1}}\\
		&\geq \frac1{4m}\cdot \sum_{i=1}^k \sum_{j=2}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j-1}}}{\mathds{1}\set{\size{\rho_{j-1,i}} \leq 0.1} \cdot \eex{\Idl_{X^{k}_{j-1}|Z^k X^k_{<j-1}}}{\gamma_{j,i} \cdot \mathds{1}\set{\gamma_{j,i} > 1}}}\\
		&\geq \frac1{16m} \sum_{i=1}^k \sum_{j=2}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j-1}}}{\mathds{1}\set{\size{\rho_{j-1,i}} \leq 0.1} \cdot 	\eex{\Idl_{X^{k}_{j-1}|Z^k X^k_{<j-1}}}{\bbeta_{j,i} \cdot \mathds{1}\set{\gamma_{j,i} > 1}}}\\
		&= \frac1{16m} \sum_{i=1}^k \sum_{j=2}^{m+1} \eex{\Idl_{Z^k X^{k}_{<j-1}}}{\xi_{j-1,i} \cdot \mathds{1}\set{\size{\rho_{j-1,i}} \leq 	0.1}}\\
		&= \frac1{16m} \sum_{i=1}^k \sum_{j=1}^{m} \eex{\Idl_{Z^k X^{k}_{<j}}}{\xi_{j,i} \cdot \mathds{1}\set{\size{\rho_{j,i}} \leq 0.1}},
	\end{align*}
	where the first inequality follows by \cref{claim:bad_events:gamma} and the fact that $\gamma_{j,i} > 1 \implies 1 \notin X_{<j,i}$, and the third one by \cref{claim:bad_events:list_of_properties}(\ref{item:bad_events:list_of_properties:4}).
\end{proof}

As a first corollary of \cref{claim:bad_events:xi}, we obtain the following.

\begin{corollary}\label{corollary:bad_events:xi:first}
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $\eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m} \xi_{j,i} \cdot \mathds{1}\set{\size{\rho_{j,i}} \leq 0.1}} \geq \zfrac{\eps k}{\lambda}$ for $\xi_{j,i} = \xi_{j,i}(Z^k X^{k}_{<j})$ and $\rho_{j,i} = \rho_{j,i}(Z^k X^{k}_{<j})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{corollary}
\begin{proof}
	Immediately follows by \cref{claim:bad_events:xi}.
\end{proof}

As a second corollary of \cref{claim:bad_events:xi}, we obtain that if $\Unf[W]$ is high enough, then most columns $i \in [k]$ have bounded sum $\sum_{j=1}^{m} \xi_{j,i}$ in expectation over $\Idl$.

\begin{corollary}\label{corollary:bad_events:xi:second}
	For any constants $\lambda > 0$ and $c \in (0,1)$ there exists a constant $\lambda' > 0$ such that if $\eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}} \geq \zfrac{\eps k}{\lambda}$ for $\xi_{j,i} = \xi_{j,i}(Z^k X^{k}_{<j})$ , then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{corollary}
\begin{proof}
	Assume that $\eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}} \geq \zfrac{\eps k}{\lambda}$ for some constant $\lambda > 0$. Observe that
	\begin{align*}
		\lefteqn{\eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}}}\\
		&= \eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c} \cdot \mathds{1}\set{\jmp^{\rho}_{i} = \infty}} + \eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}\cdot \mathds{1}\set{\jmp^{\rho}_{i} < \infty}},
	\end{align*}
	where $\jmp^{\rho}_{i} = \jmp^{\rho}_{i}(Z^k X^{(m+1) \times k})$. If $\eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}\cdot \mathds{1}\set{\jmp^{\rho}_{i} < \infty}} > \frac{\eps k}{2\lambda}$ then in particular, $\eex{\Idl}{\jumps^{\rho}(Z^k X^{(m+1)\times k})} = \eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\jmp^{\rho}_{i} < \infty}} > \frac{\eps k}{2\lambda}$ and the proof follows by \cref{claim:bad_events:main-lemma-easy-jumps}. Otherwise, $\eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c} \cdot \mathds{1}\set{\jmp^{\rho}_{i} = \infty}} \geq \frac{\eps k}{2\lambda}$. Compute
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \frac1{16m} \cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m} \xi_{j,i} \cdot \mathds{1}\set{\size{\rho_{j,i}} \leq 0.1}}\\
		&\geq \frac1{16m} \cdot \eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}\cdot \mathds{1}\set{\jmp^{\rho}_{i} = \infty}\cdot \sum_{j=1}^{m} \xi_{j,i} \cdot \mathds{1}\set{\size{\rho_{j,i}} \leq 0.1}}\\
		&= \frac1{16m} \cdot \eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}\cdot \mathds{1}\set{\jmp^{\rho}_{i} = \infty}\cdot \sum_{j=1}^{m} \xi_{j,i}}\\
		&\geq \frac{c}{16m} \cdot \eex{\Idl}{\sum_{i=1}^k \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c} \cdot \mathds{1}\set{\jmp^{\rho}_{i} = \infty}}\\
		&\geq c \cdot \frac{\eps k}{32 \lambda\cdot m}
		\implies \Unf[W] \leq e^{-c \cdot \frac{\eps k}{32 m \lambda}} \leq (1-\eps)^{\frac{\eps k}{\left(\zfrac{32 \lambda}{c}\right)\cdot m}}
	\end{align*}
	where the first inequality holds by \cref{claim:bad_events:xi} and the last one hold since $\eps \in [0,\frac12]$.
\end{proof}

The following claim is the heart of this section. It states that if $\Unf[W]$ is high enough, then in expectation (over $\Idl$), the sum of squares of all sequences' elements (Namely, $\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2$) is at most $o(\eps k)$. This later yields that for a typical column $i \in [k]$ we expect that $\sum_{j=2}^{m+1} \hbeta_{j,i}^2 \leq o(\eps)$ and then the ideas of Section~\ref{sec:bad_events:a_values:high_level_plan} follows.

\begin{claim}\label{claim:bad_events:delta_squeres}
	For any constant $\lambda > 0$ there exists a constant $\lambda' > 0$ such that if $\eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2} \geq \zfrac{\eps k}{\lambda}$ for $\hbeta_{j,i} = \hbeta_{j,i}(Z^k X^k_{<j})$, then $\Unf[W] \leq (1-\eps)^{\frac{k}{\lambda' \cdot m}}$.
\end{claim}
\begin{proof}
	Assume that $\eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2} \geq \zfrac{\eps k}{\lambda}$ for some constant $\lambda > 0$.
	If $\eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{\gamma_{j,i} > 1}} \geq \frac{\eps k}{2\lambda}$ then the proof follows since
	\begin{align*}
		\log{\frac1{\Unf[W]}}
		&\geq \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \frac{\min\set{\size{\gamma_{j,i}}, \gamma_{j,i}^2}}{4m} \cdot \mathds{1}\set{1 \notin x_{<j,i}}}\\
		&\geq \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1}  \frac{\gamma_{j,i}}{4m} \cdot \mathds{1}\set{\gamma_{j,i} > 1}}\\
		&\geq \frac1{196 m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \hbeta_{j,i}^2 \cdot 	\mathds{1}\set{\gamma_{j,i} > 1}}\\
		&\geq \frac{\eps k}{392\lambda\cdot m} \implies \Unf[W] \leq e^{-\frac{\eps k}{392\lambda\cdot m}} \leq (1-\eps)^{\frac{\eps k}{392\lambda\cdot m}},
	\end{align*}
	where the first inequality holds by \cref{claim:bad_events:gamma}, the third one holds since $\size{\hbeta_{j,i}} \leq 7$ (property \ref{item:bad_events:list_of_properties:3} of \cref{claim:bad_events:list_of_properties}) and the last one holds since $\eps \in [0,\frac12]$.
	Otherwise, it holds that
	\begin{align}\label{eq:bad_events:delta_squares:0}
		\lefteqn{\eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{\gamma_{j,i} \leq 1}}}\nonumber\\
		&= \eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{X_{j-1,i}=1}}
		+ \eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1}}\nonumber\\
		&\geq \frac{\eps k}{2\lambda}
	\end{align}
	Now, observe that
	\begin{align}\label{eq:bad_events:delta_squares:1}
		\lefteqn{\eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{X_{j-1,i}=1}}}\nonumber\\
		&= \eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{X_{j-1,i}=1} \cdot \mathds{1}\set{\Good_{j-1,i} = 1}}\nonumber\\
		&= \eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} (\xi_{j-1,i} - \frac{\gamma_{j-1,i}}{m-1})^2 \cdot \mathds{1}\set{\Good_{j-1,i} = 1}}\nonumber\\
		&\leq \eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} 2(\xi_{j-1,i}^2 + \frac{\gamma_{j-1,i}^2}{(m-1)^2}) \cdot \mathds{1}\set{\Good_{j-1,i} = 1}}\nonumber\\
		&\leq \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m-1} \xi_{j,i} \cdot \mathds{1}\set{\size{\rho_{j,i}} \leq 0.1}} + 2 \cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m-1} \gamma_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}} \cdot \mathds{1}\set{\gamma_{j,i} \leq 1}},
	\end{align}
	where the first inequality holds by the fact that $(a+b)^2 \leq 2(a^2 + b^2)$, and the last one holds since $\Good_{j-1,i} = 1 \implies \size{\gamma_{j-1,i}},\size{\rho_{j-1,i}},\xi_{j-1,i} \leq 0.1$ and since $m \geq 2$ and $\xi_{j-1,i} \geq 0$.
	Therefore, if $\eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{X_{j-1,i}=1}} \geq \frac{\eps k}{4\lambda}$, then at least one of the terms in (\ref{eq:bad_events:delta_squares:1}) must be $ \geq \frac{\eps k}{8\lambda}$ and the proof follows by \cref{corollary:bad_events:xi:first,corollary:bad_events:gamma:small}.
	Otherwise, it holds by \cref{eq:bad_events:delta_squares:0} that $\eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1}} \geq  \frac{\eps k}{4\lambda}$. Compute
	\begin{align}\label{eq:bad_events:delta_squares:main_eq}
		\lefteqn{\log{\frac1{\Unf[W]}}}\nonumber\\
		&\geq \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \frac{\min\set{\size{\gamma_{j,i}}, \gamma_{j,i}^2}}{4m}\cdot \mathds{1}\set{1 \notin X_{<j,i}}}\nonumber\\
		&\geq \frac1{4m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m+1} \gamma_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}} \cdot \mathds{1}\set{\gamma_{j,i} \leq 1} \cdot \mathds{1}\set{\Good_{j-1,i} = 1}}\nonumber\\
		&\geq \frac1{4m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} (\frac1{10} \hbeta_{j,i}^2 - \gamma_{j-1,i}^2 - \xi_{j-1,i} - 3 \rho_{j-1,i}^2) \cdot \mathds{1}\set{1 \notin X_{<j,i}} \cdot \mathds{1}\set{\gamma_{j,i} \leq 1} \cdot \mathds{1}\set{\Good_{j-1,i} = 1}}\nonumber\\
		&\geq \frac{1}{160 m} \eex{\Idl}{\sum_{i=1}^k \sum_{j=2}^{m+1} \hbeta_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1}}\\
		&- \frac1{4m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m} \gamma_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\gamma_{j,i} \leq 1}}\nonumber\\
		&- \frac3{4m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m} \rho_{j,i}^2 \cdot \mathds{1}\set{1 \notin X_{<j,i}}\cdot \mathds{1}\set{\rho_{j,i} \leq 1}}\nonumber\\
		&- \frac1{4m}\cdot \eex{\Idl}{\sum_{i=1}^k \sum_{j=1}^{m} \xi_{j,i} \cdot \mathds{1}\set{\size{\rho_{j,i}} \leq 0.1}},\nonumber
	\end{align}
	where the first inequality holds by \cref{claim:bad_events:gamma}, the second one holds since $\Good_{j-1,i} = 1 \implies \size{\gamma_{j-1,i}} \leq 0.1$ and the third one holds by \cref{claim:bad_events:list_of_properties} (property~\ref{item:bad_events:list_of_properties:6}) since $\Good_{j-1,i} = 1 \implies \size{\rho_{j-1,i}},\xi_{j-1,i} \leq 0.1$. By assumption, the first term in \cref{eq:bad_events:delta_squares:main_eq} is at least $\frac{\eps k}{4\lambda}$. Therefore, there are two options: The first option is that the sum of terms in (\ref{eq:bad_events:delta_squares:main_eq})$ \geq \frac{\eps k}{8\lambda} \implies \Unf[W] \leq e^{-\frac{\eps k}{8\lambda}} \leq (1-\eps)^{\frac{\eps k}{16\lambda}}$. The second option is that at least one of the negative terms in (\ref{eq:bad_events:delta_squares:main_eq}) has absolute value $\geq \frac{\eps k}{24\lambda}$, and then the proof follows by \cref{corollary:bad_events:gamma:small,claim:bad_events:rho:small,corollary:bad_events:xi:first}.
\end{proof}

The following claim focuses on ``good'' columns, \ie columns $i \in [k]$ with bounded sums $\set{\sum_{j'=2}^j \hbeta_{j',i}}_{j=2}^{m+1}$ and with small values of $\set{\gamma_{j,i}}_{j=1}^{m+1}$, $\set{\rho_{j,i}}_{j=1}^{m+1}$ and $\set{\sum_{j'=1}^j \xi_{j',i}}_{j=1}^{m}$. For these columns, the claim connects the sums $\set{\sum_{j'=2}^j \hbeta_{j',i}}_{j =2}^{m+1}$ into the required products $\set{\prod_{j'=2}^{j}(1 + \bbeta_{j',i})}_{j =2}^{m+1}$ by showing that they are indeed bounded in an interval of constants. Along with assuming  that the first two terms of $\aval_{j,i}$ are $\approx 1$, the claim concludes that for such columns it holds that the values of $\set{\aval_{j,i}}_{j=1}^{m+1}$ are indeed bounded.

\begin{claim}\label{claim:bad_events:from_tdelta_to_a}
	There exists a constant $c \in (0,0.1)$ such that for any $z^k x^{(m+1) \times k} \in \Supp(\Idl_{Z^k X^{(m+1) \times k}})$ and $i \in [k]$, it holds that $i \in \GSet^{\aval}_{z^k x^{(m+1) \times k}}$ if all the following conditions hold:
	\begin{enumerate}
		\item $\frac{\Unf_{Z_{i}}(z_i)}{\Idl_{Z_{i}}(z_i)} \in 1 \pm c$, and
		\item $\frac{\Idl_{X_{1,i} | Z^k}(1 | z^k)}{\Idl_{X_{1,i} | Z_{i}}(1 | z_{i})} \in 1 \pm c$, and
		\item $i \in \GSet^{\gamma}_{z^k x^{(m+1) \times k}} \bigcap \GSet^{\rho}_{z^k x^{(m+1) \times k}}$, and
		\item $\sum_{j=1}^{m} \xi_{j,i}(z^k x^k_{<j}) \leq c$, and
		\item $\sum_{j=2}^{m+1} \hbeta^2_{j,i}(z^k x^k_{<j}) \leq c$, and
		\item $\max\set{\size{\sum_{j'=2}^j \hbeta_{j',i}(z^k x^k_{<j})}}_{j=2}^{m+1} \leq c$.
	\end{enumerate}
\end{claim}
\begin{proof}
	Fix $j \in [m+1]$ and recall that
	\begin{align*}
		\aval_{j,i}
		&= \frac{\Unf_{Z_{i}}(z_i)}{\Idl_{Z_{i}}(z_i)} \cdot \frac{\Idl_{X_{1,i} | Z^k}(1 | z^k)}{\Idl_{X_{1,i} | Z_{i}}(1 | z_{i})} \cdot \prod_{j'=2}^{j}(1 + \bbeta_{j',i})
	\end{align*}

	By assumption, it holds that $\size{\gamma_{j'-1,i}},\size{\rho_{j'-1,i}}, \sum_{j'=2}^j \xi_{j'-1,i} \leq 0.1$ for any $j' \in [j]\setminus \set{1}$. In particular, this yields that for any such $j'$ it holds that
	\begin{enumerate}[a.]
		\item $\hbeta_{j',i} = \bbeta_{j',i} + \xi_{j'-1,i} - \bbeta_{j',i}^U + \mu_{j'-1,i}$.
		\item $\bbeta^U_{j',i} = \frac1{m-1}$.
		\item $\bbeta_{j',i} = \frac{1 + \gamma_{j',i}}{1+\rho_{j'-1,i}}\cdot \frac{m}{m-1} - 1 \geq \frac{0.9}{1.1} \cdot \frac{m}{m-1} - 1 \geq -0.2$.
	\end{enumerate}
	Using the above observations, we prove that $\aval_{j,i} \in [0.01,10]$.
	Note that the upper bound holds since
	\begin{align*}
		\aval_{j,i}
		&\leq (1+c)^2 \cdot e^{\sum_{j'=2}^j \bbeta_{j',i}}\\
		&= (1+c)^2 \cdot e^{\sum_{j'=2}^j (\hbeta_{j',i} - \xi_{j'-1,i} + \bbeta^U_{j',i} - \mu^U_{j'-1,i})}\\
		&\leq (1+c)^2 \cdot e^{c - 0 + \frac{j-1}{m-1} + \frac{0.1 \cdot (j-1)}{m-1}}\\
		&\leq (1+c)^2 \cdot e^{c + 2.2}
	\end{align*}

	and the lower bound holds since
	\begin{align*}
		\aval_{j,i}
		&\geq (1-c)^2 \cdot e^{\sum_{j'=1}^j \bbeta_{j',i}}\cdot e^{-\sum_{j'=1}^j \bbeta^2_{j',i}}\\
		&= (1-c)^2 \cdot e^{\sum_{j'=2}^j (\hbeta_{j',i} - \xi_{j'-1,i} + \bbeta^U_{j',i} - \mu^U_{j'-1,i})}\cdot e^{-0.6 \cdot \sum_{j'=1}^j (\hbeta_{j',i} - \xi_{j'-1,i} + \bbeta^U_{j',i} - \mu^U_{j'-1,i})^2}\\
		&\geq (1-c)^2 \cdot e^{-c -c + \frac{j-1}{m-1} -\frac{0.1 \cdot (j-1)}{m-1}} \cdot e^{0.6 \cdot \paren{-6 \sum_{j'=1}^j\left(\hbeta_{j',i}^2 + \xi_{j'-1,i}^2 + (\frac{\gamma_{j'-1,i}}{m-1})^2\right) - 2 \sum_{j'=1}^j (\bbeta^U_{j',i})^2}}\\
		&\geq (1-c)^2 \cdot e^{-2c} \cdot e^{-4 \left(c + c^2 + (\frac{0.1}{m-1})^2\cdot (j-1)\right) - 4}\\
		&= (1-c)^2 \cdot e^{-6c-4c^2-4.08},
	\end{align*}
	where the first inequality holds by the fact that $1+x \geq e^{x-0.6 x^2}$ for $x \geq -0.2$, the second one holds by the fact that $(a+b+c+d)^2 \leq 2\paren{(a+b+c)^2 + d^2} \leq 6(a^2 + b^2 + c^2) + 2d^2$ and the last one holds since $\sum_{j'=2}^{j} \hbeta^2_{j',i} \leq c$ and $\sum_{j'=1}^{j} \xi_{j',i}^2 \leq \sum_{j=1}^{m} \xi_{j,i} \leq c$ and $\sum_{j'=1}^j (\bbeta^U_{j',i})^2 \leq \frac{m}{(m-1)^2} \leq 2$ and $(\frac{0.1}{m-1})^2\cdot (j-1) \leq \frac{0.01 m}{(m-1)^2} \leq 0.02$.
	By taking $c=0.01$ we obtain that $\aval_{j,i} \in [0.01,10]$, as required.
\end{proof}


As a corollary of all the claims of this section, we are finally ready to prove \cref{claim:bad_events:main-lemma-hard-jumps}.

\paragraph{Putting it Together}\label{sec:bad_events:hard-jumps:putting-it-together}

\begin{corollary}[Restatement of \cref{claim:bad_events:main-lemma-hard-jumps}]
	\MainLemmaHardJumps
\end{corollary}

\begin{proof}
	Let $c$ be the constant from \cref{claim:bad_events:from_tdelta_to_a}. Observe that \cref{claim:bad_events:from_tdelta_to_a} implies that
	\begin{align*}
		\mathds{1}\set{\jmp^{\aval}_i < \infty}
		&\leq \mathds{1}\set{\frac{\Unf_{Z_{i}}(z_i)}{\Idl_{Z_{i}}(z_i)} \notin 1 \pm c}
		+  \mathds{1}\set{\frac{\Idl_{X_{1,i} | Z^k}(1 | z^k)}{\Idl_{X_{1,i} | Z_{i}}(1 | z_{i})} \notin 1 \pm c}\\
		&+ \mathds{1}\set{\jmp^{\size{\gamma} > 0.1} < \infty}
		+ \mathds{1}\set{\jmp^{\size{\rho} > 0.1} < \infty}
		+ \mathds{1}\set{\sum_{j=1}^{m} \xi_{j,i} > c}\\
		&+ \mathds{1}\set{\sum_{j=2}^{m+1} \hbeta^2_{j,i} > c}
		+ \mathds{1}\set{\max\set{\size{\sum_{j'=2}^j \hbeta_{j',i}}}_{j=2}^{m+1} > c}
	\end{align*}
	Therefore, by assumption (recall that $\jumps^{\aval}(Z^k X^{(m+1) \times k}) = \sum_{i=1}^{k} \mathds{1}\set{\jmp^{\aval}_i < \infty}$), when summing over $i \in [k]$ and taking expectation over $\Idl$, 
	the sum of all the right side terms is at least  $\frac{\eps k}{\lambda}$. If one of the first five terms have expected sum $\geq \frac{\eps k}{10 \lambda}$, then the proof follows by \cref{claim:bad_events:a_first_term,claim:bad_events:a_sec_term,corollary:bad_events:gamma:large-and-J,corollary:bad_events:rho:large-and-J,corollary:bad_events:xi:second}. Otherwise, it holds that
	\begin{align}\label{eq:bad_events:Ja:1}
		\eex{\Idl}{\sum_{i=1}^k \left(\mathds{1}\set{\sum_{j=2}^{m+1} \hbeta^2_{j,i} > c} + \mathds{1}\set{\max\set{\size{\sum_{j'=2}^j \hbeta_{j,i}}}_{j=1}^{m+1} > c}\right)} \geq \frac{\eps k}{2 \lambda}
	\end{align}
	 For $i \in [k]$, let $q_i =\eex{\Idl}{\sum_{j=2}^{m+1} \hbeta_{j,i}^2}$. Note that \cref{claim:bad_events:list_of_properties} (property~\ref{item:bad_events:list_of_properties:2}) yields that the sequence $\set{\hbeta_{j,i}(Z^k X^{k}_{<j})}_{j=2}^{m+1}$ is a martingale difference sequence with respect to $\set{\Idl_{X^k_j | Z^k X^k_{<j}}}_{j=1}^{m}$ (for any fixing of $Z^k$). Therefore, \cref{fact:prelim:martingales:week_concent} yields that
	$\Idl\left[\max\set{\size{\sum_{j'=2}^j \hbeta_{j,i}}}_{j=1}^k > c\right] \leq \zfrac{q_i}{c^2}$ which implies that
	\begin{align}\label{eq:bad_events:Ja:partial_sums}
		\eex{\Idl}{\mathds{1}\set{\max\set{\size{\sum_{j'=2}^j \hbeta_{j,i}}}_{j=2}^{m+1} > c}} \leq \zfrac{q_i}{c^2}.
	\end{align}
	Moreover, by Markov inequality, it holds that $\Idl\left[\sum_{j=2}^{m+1} \hbeta_{j,i}^2(Z^k X^k_{<j}) > c\right] \leq \zfrac{q_i}{c}$ which implies that
	\begin{align}\label{eq:bad_events:Ja:sum_of_squares}
		\eex{\Idl}{\mathds{1}\set{\sum_{j=2}^{m+1} \hbeta^2_{j,i} > c}} \leq \zfrac{q_i}{c}
	\end{align}
	Hence, \cref{eq:bad_events:Ja:1,eq:bad_events:Ja:partial_sums,eq:bad_events:Ja:sum_of_squares} yields that
	\begin{align*}
		\left(\zfrac1{c} + \zfrac1{c^2}\right) \sum_{i=1}^k q_i 
		&\geq \eex{\Idl}{\sum_{i=1}^k \left(\mathds{1}\set{\sum_{j=2}^{m+1} \hbeta^2_{j,i} > c} + \mathds{1}\set{\max\set{\size{\sum_{j'=2}^j \hbeta_{j,i}}}_{j=1}^{m+1} > c}\right)}\\
		&\geq \frac{\eps k}{2 \lambda}\\
		&\implies \eex{\Idl}{\sum_{j=2}^{m+1} \sum_{i=1}^k \hbeta_{j,i}^2} = \sum_{i=1}^k q_i \geq  \frac{\eps k}{2 \lambda\cdot (\zfrac1{c} + \zfrac1{c^2})}
	\end{align*}
	and the proof follows by \cref{claim:bad_events:delta_squeres}.
\end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "TightPR"
%%% End:

